Dynamic DFS Tree in Undirected Graphs: breaking the $O(m)$ barrier

Depth first search (DFS) tree is a fundamental data structure for solving various problems in graphs. It is well known that it takes $O(m+n)$ time to build a DFS tree for a given undirected graph $G=(V,E)$ on $n$ vertices and $m$ edges. We address the problem of maintaining a DFS tree when the graph is undergoing {\em updates} (insertion and deletion of vertices or edges). We present the following results for this problem. (a) Fault tolerant DFS tree: There exists a data structure of size ${O}(m ~polylog~ n)$ such that given any set ${\cal F}$ of failed vertices or edges, a DFS tree of the graph $G\setminus {\cal F}$ can be reported in ${O}(n|{\cal F}| ~polylog~ n)$ time. (b) Fully dynamic DFS tree: There exists a fully dynamic algorithm for maintaining a DFS tree that takes worst case ${O}(\sqrt{mn} ~polylog~ n)$ time per update for any arbitrary online sequence of updates. (c) Incremental DFS tree: Given any arbitrary online sequence of edge insertions, we can maintain a DFS tree in ${O}(n ~polylog~ n)$ worst case time per edge insertion. These are the first $o(m)$ worst case time results for maintaining a DFS tree in a dynamic environment. Moreover, our fully dynamic algorithm provides, in a seamless manner, the first deterministic algorithm with $O(1)$ query time and $o(m)$ worst case update time for the dynamic subgraph connectivity, biconnectivity, and 2-edge connectivity.

==> New folder/abstract.tex <==
Depth first search (DFS) tree is a fundamental data structure for solving various problems in graphs. It is well known that it takes $O(m+n)$ time to build a DFS tree for a given undirected graph $G=(V,E)$ on $n$ vertices and $m$ edges. We address the problem of maintaining a DFS tree when the graph is undergoing {\em updates} (insertion and deletion of vertices or edges). We present the following results for this problem.

\begin{enumerate}
\item {\em Fault tolerant DFS tree}:
There exists a data structure of size $\tilde{O}(m)$ \footnote{$\tilde{O}()$ hides the poly-logarithmic factors.} such that given any set ${\cal F}$ of failed vertices or edges, a DFS tree of the graph $G\setminus {\cal F}$ can be reported in $\tilde{O}(n|{\cal F}|)$ time. 

\item {\em Fully dynamic DFS tree}:
There exists a fully dynamic algorithm for maintaining a DFS tree that takes worst case $\tilde{O}(\sqrt{mn})$ time per update  for any arbitrary online sequence of updates.

\item {\em Incremental DFS tree}:
There exists an incremental algorithm for maintaining a DFS tree that takes worst case $\tilde{O}(n)$ time per update for any arbitrary online sequence of edge insertion.
\end{enumerate}

These are the first $o(m)$ worst case time results for maintaining a DFS tree in a dynamic environment. Moreover, our fully dynamic algorithm provides, in a seamless manner, the first deterministic algorithm with $O(1)$ query time and $o(m)$ worst case update time for connectivity, biconnectivity, and 2-edge connectivity in the dynamic subgraph model. 

\noindent
\textbf{Keywords: }
  Depth First Search, DFS, Dynamic Graph Algorithm





==> New folder/appn.tex <==
%\label{sec:apnIntro}
%Our fully dynamic algorithm for maintaining a DFS tree can  be used to solve 
%various dynamic graph problems such as dynamic subgraph connectivity, bi-connectivity and 2 edge connectivity.
%Note that these problems are solved trivially using DFS tree in the static setting.
%The solution of dynamic subgraph connectivity follows seamlessly from our fully dynamic algorithm as follows.
%As mentioned in Section \ref{sec:prelim}, we maintain a DFS tree rooted at a dummy vertex $r$, such that
%the subtrees hanging from its children corresponds to connected components of the graph. 
% %we maintain a dummy vertex $r$ as the root of the DFS tree.
%%The DFS tree for each component is a child subtree of $r$. 
%Hence the connectivity query for any two vertices 
%can be answered by comparing their ancestors at depth two (i.e. children of $r$).
%This information can be stored for each vertex and updated whenever the DFS tree is updated.
%Thus we have a data structure for subgraph connectivity with worst case $\tilde{O}(\sqrt{mn})$ update time 
%and $O(1)$ query time. Similarly our algorithm can be used to solve dynamic subgraph bi-connectivity and  
%2-edge connectivity in the same time bounds. For details refer to Appendix \ref{sec:appn}.


\section{Applications}
\label{sec:appn}
Our fully dynamic algorithm for maintaining a DFS tree can  be used to solve 
various dynamic graph problems such as dynamic subgraph connectivity, biconnectivity and 2-edge connectivity.
Note that these problems are solved trivially using a DFS tree in the static setting.
%We now describe some applications of our fully dynamic DFS algorithm.
%As described in Section \ref{sec:apnIntro}, our fully dynamic DFS algorithm seamlessly 
%gives a solution  for solving dynamic subgraph connectivity.
Let us now describe the importance of our result in the light of the existing results for these problems.
%Note that all the results mentioned in the following section are restricted to  
%deterministic algorithms.


%\subsubsection*{Dynamic subgraph connectivity}
\subsection{Existing Results}
The dynamic subgraph connectivity problem is defined as follows. Given
an undirected graph, the status of any vertex can be switched between  
{\it active} and {\it inactive} in an update. 
For any online sequence of updates interspersed with queries, 
the goal is to efficiently answer each connectivity queries 
on the subgraph induced by the active vertices. 
%The goal is to efficiently answer any online sequence of connectivity queries 
%on the subgraph induced by the active vertices. 
%The goal is to efficiently answer any online connectivity query on the subgraph induced by the 
%active vertices. 
This problem can be solved by using dynamic connectivity
data structures \cite{EppsteinGIN97,Frederickson85,HolmLT01,KapronKM13} that answer
connectivity queries under an online sequence of edge updates. This is 
because switching the state of a vertex is equivalent to $O(n)$ edge 
updates. Chan \cite{Chan06} introduced this problem and showed that it 
can be solved more efficiently. He gave an algorithm using FMM (fast 
matrix multiplication) that achieves $O(m^{0.94})$ amortized update time 
and $\tilde{O}(m^{1/3})$ query time. Later Chan et al. \cite{ChanPR08} 
presented a new algorithm that improves the amortized update time to 
$\tilde{O}(m^{2/3})$. 
%Further they established a lower bound of $\Omega(\sqrt{m})$ time per update. 
%Duan \cite{Duan10} presented an algorithm with $O(m^{4/5})$ worst case update time
%and $O(m^{1/5})$ update time, improving the worst case bounds for the problem.  
They also mentioned the following 
among the open problems.

\begin{enumerate}
\item
Is it possible to achieve constant query time with worst case sublinear ($o(m)$)
update time ?
\item
Can non trivial updates be obtained for richer queries such as counting
the number of connected components ?
\end{enumerate}

Duan \cite{Duan10} partially answered the first question affirmatively but at the
expense of a much higher update time and non-constant query time. He presented an 
algorithm with $O(m^{4/5})$ worst case update time
and $O(m^{1/5})$ query time, improving the worst case bounds for the problem.
Kapron et al. \cite{KapronKM13} presented a randomized algorithm for fully dynamic connectivity
which takes $\tilde{O}(1)$ time per update and answers the query correctly with high probability in $\tilde{O}(1)$ time, 
giving a Monte Carlo algorithm for subgraph connectivity with worst case $\tilde{O}(n)$ update time. 
Thus, their result answered the first question in a randomized setting.
However, in the deterministic setting both these questions were still open.
Our result answers both these questions affirmatively for the deterministic setting as well. 
Our fully dynamic algorithm directly provides an 
$\tilde{O}(\sqrt{mn})$ update time and $O(1)$ query time algorithm for 
the dynamic subgraph connectivity problem. Our algorithm maintains the
number of connected components simply as a byproduct. In fact, our fully dynamic
algorithm for DFS tree solves a generalization of dynamic subgraph connectivity 
- in addition to just switching the status of vertices, it allows insertion of 
new vertices as well. 
Hence the existing results offer different trade-offs between the update time and the query time, 
and differ on the types (amortized or worst case) of update time and the types (deterministic or randomized) of query time. 
Our algorithm, in particular, improves the deterministic worst 
case bounds for the problem (see Figure \ref{figure:subGraph}).
%
%Exploiting the rich structure of DFS tree, we also obtain 
%$\tilde{O}(\sqrt{mn})$ update time algorithms for dynamic subgraph 
%bi-connectivity and dynamic subgraph 2-edge connectivity in a seamless 
%manner. Figure \ref{figure:subGraph} illustrates our results and the 
%existing results in the right perspective. A variant of dynamic 
%subgraph connectivity problem has been studied by 
%Patrascu and Thorup \cite{PatrascuT07}. For any $k$ edge failures,
%their data structure takes $\tilde{O}(k)$ update time such that
%any subsequent connectivity query can be answered in $O(\log\log n)$ time.
%Later Duan and Pettie \cite{DuanP10} presented a data structure for vertex
%failures. For any $k$ vertex failures, their data structure takes 
%$\tilde{O}(k^6)$ update time and answers any subsequent 
%connectivity query in $O(k)$ time.
%
%The connectivity problem 
%have also been studied in the fault tolerant model by Patrascu and Thorup
%\cite{PatrascuT07} for edge failures and by Duan and Pettie \cite{DuanP10} 
%for vertex failures. The subgraph connectivity problem have also been studied
%in the fault tolerant model. Patrascu and Thorup \cite{PatrascuT07} showed 
%that one can answer connectivity queries after $d$ edge failures using 
%$\tilde{O}(d)$ update time. Later Duan and Pettie \cite{DuanP10} improved 
%this update time for $d$ vertex failures to $\tilde{O}(d^6)$. 
Further, unlike all the previous algorithms for dynamic subgraph connectivity, which use heavy 
machinery of existing dynamic algorithms, our algorithm is arguably much 
simpler and self contained. 

%%%%%%%% SPACE VERSION
%\begin{figure}[h!]
%\centering
%\def\arraystretch{0.6}
%\begin{tabular}{| m{4.5cm} | m{3.5cm} | m{2cm} | m{1.5cm} |}
%\hline
% {\bf References }							& {\bf Update Time} 					& {\bf Query Time} 		& {\bf Space} 			\\ \hline
%Frederickson \cite{Frederickson85} (1985), 
%Eppstein et. al \cite{EppsteinGIN97} (1997)\hfill$\dagger$& $O(n\sqrt{n})$  					& $O(1)$ 				& $O(m)$  				\\ \hline
%Holm et al. \cite{HolmLT01} (2001)\hfill$*\dagger$  		& $\tilde{O}(n)$ amortized  			& $\tilde{O}(1)$ 		& $O(m)$  				\\ \hline
%Chan  \cite{Chan06} (2006) 					& $\tilde{O}(m^{0.94})$ amortized	& $\tilde{O}(m^{1/3})$ 	& $\tilde{O}(m)$  		\\ \hline
%Chan et al. \cite{ChanPR08} (2008) 			& $\tilde{O}(m^{2/3})$ amortized		& $\tilde{O}(m^{1/3})$ 	& $\tilde{O}(m^{4/3})$ 	\\ \hline
%Duan \cite{Duan10} (2010) 					& $\tilde{O}(m^{2/3})$ amortized		& $\tilde{O}(m^{1/3})$ 	& $\tilde{O}(m)$  		\\ \hline
%Duan \cite{Duan10} (2010) 					& $\tilde{O}(m^{4/5})$ 				& $\tilde{O}(m^{1/5})$ 	& $\tilde{O}(m)$  		\\ \hline
%Kapron et al. \cite{KapronKM13} (2013)		& $\tilde{O}(n)$ 					& $\tilde{O}(1)$ w.h.p.	& $\tilde{O}(m)$  		\\ \hline
%{\bf New\hfill $*\dagger$} 								& $\tilde{O}(\sqrt{mn})$ 			& $O(1)$ 				& $\tilde{O}(m)$  		\\ \hline
%\end{tabular}
%\caption{Current-state-of-the-art of the algorithms for the dynamic subgraph 
%connectivity.} % $(*)$ and $(\dagger)$ indicates that the result also solves subgraph bi-connectivity and 2-edge connectivity respectively.}
%\label{figure:subGraph}
%\end{figure}


\begin{figure}[!ht]
\centering
\def\arraystretch{0.6}
\begin{tabular}{| m{4.5cm} | m{3.5cm} | m{2.2cm} |}
\hline
 {\bf References }							& {\bf Update Time} 					& {\bf Query Time} 		\\ \hline
Frederickson \cite{Frederickson85} (1985), 
Eppstein et. al \cite{EppsteinGIN97} (1997)	& $O(n\sqrt{n})$  					& $O(1)$ 	\\ \hline
Holm et al. \cite{HolmLT01} (2001)			& $\tilde{O}(n)$ amortized  			& $\tilde{O}(1)$ 		\\ \hline
Chan  \cite{Chan06} (2006) 					& $\tilde{O}(m^{0.94})$ amortized	& $\tilde{O}(m^{1/3})$ 	\\ \hline
Chan et al. \cite{ChanPR08} (2008) 			& $\tilde{O}(m^{2/3})$ amortized		& $\tilde{O}(m^{1/3})$ 	\\ \hline
%Duan \cite{Duan10} (2010) 					& $\tilde{O}(m^{2/3})$ amortized		& $\tilde{O}(m^{1/3})$ 	\\ \hline
Duan \cite{Duan10} (2010) 					& $\tilde{O}(m^{4/5})$ 				& $\tilde{O}(m^{1/5})$ 	\\ \hline
Kapron et al. \cite{KapronKM13} (2013)		& $\tilde{O}(n)$ 					& $\tilde{O}(1)$ \newline(Monte Carlo)\\ \hline
{\bf New\hfill } 								& $\tilde{O}(\sqrt{mn})$ 			& $O(1)$ 	\\ \hline
\end{tabular}
\caption{Current-state-of-the-art of the algorithms for the dynamic subgraph 
connectivity.} % $(*)$ and $(\dagger)$ indicates that the result also solves subgraph bi-connectivity and 2-edge connectivity respectively.}
\label{figure:subGraph}
\end{figure}



Exploiting the rich structure of DFS trees, we also obtain 
$\tilde{O}(\sqrt{mn})$ update time algorithms for dynamic 
biconnectivity and dynamic 2-edge connectivity under vertex updates in a seamless 
manner. These problems have mainly been studied in the dynamic setting under edges updates.
Some of these results also allow insertion and deletion of isolated vertices. Our result, on the other
hand does not impose any such restriction on insertion or deletion of vertices.
Figure \ref{figure:subGraphB2E} illustrates our results and the existing results in the right perspective.
We now describe how our algorithm can be used to solve these problems.

\begin{figure}[h!]
\centering
\def\arraystretch{0.6}
\begin{tabular}{| m{4.5cm} | m{3.5cm} | m{2cm} | m{1.5cm} |}
\hline
{\bf References }							& {\bf Update Time} 					& {\bf Query Time} 		\\ \hline
Frederickson \cite{Frederickson85} (1985), 
Eppstein et. al \cite{EppsteinGIN97} (1997)\hfill$\dagger$& $O(n\sqrt{n})$  					& $O(1)$		\\ \hline
Henzinger \cite{Henzinger00} (2000)\hfill$*$				& $\tilde{O}(n\sqrt{n})$				& $O(1)$		\\	\hline
Holm et al. \cite{HolmLT01} (2001)\hfill$*\dagger$  		& $\tilde{O}(n)$ amortized  			& $\tilde{O}(1)$ \\ \hline
{\bf New\hfill $*\dagger$} 								& $\tilde{O}(\sqrt{mn})$ 			& $O(1)$ 	\\ \hline
\end{tabular}
\caption{Current-state-of-the-art of the algorithms for the dynamic biconnectivity $(*)$ and dynamic 2-edge connectivity $(\dagger)$ under vertex updates. }
%connectivity. $(*)$ and $(\dagger)$ indicates that the result also solves subgraph bi-connectivity and 2-edge connectivity respectively.}
\label{figure:subGraphB2E}
\end{figure}


\subsection{Algorithm}
The solution of dynamic subgraph connectivity follows seamlessly from our fully dynamic algorithm as follows.
As mentioned in Section \ref{sec:prelim}, we maintain a DFS tree rooted at a dummy vertex $r$, such that
the subtrees hanging from its children corresponds to the connected components of the graph. 
 %we maintain a dummy vertex $r$ as the root of the DFS tree.
%The DFS tree for each component is a child subtree of $r$. 
Hence, the connectivity query for any two vertices 
can be answered by comparing their ancestors at depth two (i.e. children of $r$).
This information can be stored for each vertex and updated whenever the DFS tree is updated.
Thus, we have a data structure for subgraph connectivity with worst case $\tilde{O}(\sqrt{mn})$ update time 
and $O(1)$ query time.
% Similarly our algorithm can be used to solve dynamic subgraph bi-connectivity and  
%2-edge connectivity in the same time bounds. For details refer to Appendix \ref{sec:appn}.
%
%\subsubsection*{Dynamic subgraph bi-connectivity and 2 edge-connectivity}
Our fully dynamic DFS algorithm can be extended to solve fully dynamic biconnectivity 
and 2-edge connectivity under %both edge updates and 
vertex updates as follows. 

A set $S$ of vertices in a graph is called a {\em biconnected component} if it is a maximal set of vertices 
such that on failure of any vertex $w$ in $S$, the vertices of $S\setminus\{w\}$ 
remains connected. Similarly, a set $S$ is said to be {\em 2-edge connected component} if it is a
maximal set of vertices such that the failure of any edge with both endpoints in $S$
does not disconnect any two vertices in $S$. 
%The goal is to maintain a data 
%structure that can efficiently answer the queries of biconnectivity and 2-edge 
%connectivity in the dynamic setting.
The biconnectivity and 2-edge connectivity queries can be answered easily by finding \emph{articulation points} and 
\emph{bridges} of the graph. It can be shown \cite{CormenLRS09} that two vertices 
belong to same biconnected component if and only if
the path connecting them in a DFS tree of the graph 
%DFS tree path between them 
does not pass through any \emph{articulation point}. 
Similarly, two vertices belong to same 2-edge connected component if and only if 
the path connecting them in a DFS tree of the graph 
%the DFS tree path between them 
does not have a \emph{bridge}.
An articulation point and a bridge of a graph can be defined as follows:
\begin{definition}
Given a graph $G=(V,E)$, a vertex $v\in V$ is called an articulation point of $G$ 
if there exist a pair of vertices $x,y\in V$ such that every path between $x$ 
and $y$ in $G$ passes through $v$.
\end{definition}

\begin{definition}
Given a graph $G=(V,E)$, an edge $e\in E$ is called a bridge of $G$ if there exist
a pair of vertices $x,y\in V$ such that every path between $x$ and $y$ in $G$ 
passes through $e$.
\end{definition}

The articulation points and bridges of a graph can be easily computed by using DFS 
traversal of the graph. Given a DFS tree $T$ of an undirected graph $G$, we can 
index the vertices in the order they are visited by the DFS traversal. This index is 
called the \emph{DFN number} of the vertex. The \emph{high number} of a vertex $v$ 
is defined as the lowest DFN number vertex from which there is an edge incident to 
$T(v)$. Now, any non-root vertex $v$ will be an articulation point of the graph if 
high number of at least one of its children is equal to $DFN(v)$. The root $r$ of 
the DFS tree $T$ will be an articulation point if it has more than one child.
An edge $(x,y)$ of the DFS tree, where $x=par(y)$,  will be a bridge if 
the high number of $y$ is $DFN(x)$ and the high number of 
each child of $y$ (if any) is equal to $DFN(y)$. 
%either $y$
%is a leaf node with high number of $y$ equal to $DFN(y)$, or the high number of 
%each child of $y$ is equal to $DFN(y)$. 
Thus,
given the high number of each vertex in the DFS tree, the articulation points and
bridges can be determined in $O(n)$ time.


We can augment our fully dynamic 
DFS algorithm with an additional procedure to compute high number of each vertex using the same
time bounds. %in $O(nk\log^4 n)$ time.
For this we show that given any set of $k$ updates to graph $G$, 
while computing the new tree $T^*$ we also compute the high number of each vertex %can also be computed 
in $O(nk\log^4 n)$ time.
%We now show that given any set of $k$ updates to graph $G$, we can not only construct
%the new tree $T^*$, but also compute high number of each vertex in $O(nk\log^4 n)$ time.
%We now show that if there are $k$ updates to $G$, then we can not only construct
%the new tree $T^*$ in $O(nk\log^4 n)$ time, but also compute high point of each 
%vertex in the same time bound. 
For each vertex $x$, let $a(x)$ denote the highest 
ancestor of $x$ in $T^*$ such that $(x,a(x))$ is an edge in $G+U$. Note that if 
$(x,a(x))$ is a newly added edge, then it can be easily computed by scanning all 
the new edges added to the graph. This is due to fact that the total number of new 
edges added to $G$ is bounded by $nk$. So we restrict ourselves to the case when 
$(x,a(x))$ was originally present in the graph $G$. 
Recall that our algorithm computes $T^*$ by attaching paths to the partially grown tree. 
Let $P_t$ and $P_p$ be the set of paths attached to $T^*$ (during its construction) that originally 
belonged to $\TT$ and $\PP$ respectively. Further, path halving ensures that the size of $P_p$ is 
bounded by $k \log n$.
%Recall that our algorithm computed
%$T^*$ by attaching paths to the partially grown tree. Let $P_t$ be the set of paths 
%attached to $T^*$ (during its construction) that originally belonged to some tree 
%in set $\TT$. Similarly, let $P_p$ be the set of paths attached to $T^*$ that 
%originally belonged to some path in set $\PP$. Note that path halving ensures that 
%the size of $P_p$ is bounded by $k \log n$. 
For each path $p_0\in P_t\cup P_p$, let $H(p_0)$ denote the
vertex in $p_0$ that is closest to $r$ in $T^*$.

%We now give an 
%$O(nk\log^4 n)$ time algorithm for constructing a subset $A(x)$ of neighbors of $x$ 
%such that the following condition holds.

We now present the procedure for constructing a subset $A(x)$ of neighbors of $x$
while computing $T^*$ in $O(nk\log^4 n)$ time,  
%algorithm for constructing a subset $A(x)$ of neighbors of $x$ 
such that the following condition holds.

\begin{itemize}
 \item For a vertex $x$, if $a(x)\notin A(x)$, then there is some descendant
 $y$ of $x$ in $T^*$ such that $a(x)\in A(y)$.
\end{itemize}

It is easy to see that if we get such an $A(x)$ for each $x$,
then high number of each vertex can be computed easily by processing the vertices of $T^*$
in bottom-up manner. 
Now, depending upon whether paths containing $x$ and $a(x)$ belong
to set $P_p$ or $P_t$, we can have different cases described as follows.

%We show the construction of set $A(x)$ along with the case it handles in 
%following four steps.

\begin{figure}[!ht]
\centering
\includegraphics[width=.95\textwidth]{Figures/biconnec.pdf}
\caption{(i) Before the beginning of algorithm vertex $x$ belongs to
tree $T_0\in \TT$, $z$ is the highest ancestor of $x$ in $T_0$ such that
$(x,z)$ is an edge.
(ii) The partitioning changes as the algorithm proceeds, $T_1(\in\TT)$ 
is the tree containing vertex $z$ just before it is attached to $T^*$.
(iii) A path containing vertex $z$ (i.e. $p_z$) is extracted from $T_1$
and attached to $T^*$. If $a(x)$ belongs to $T_0$, then it is the highest neighbor of $x$ in $p_z$.}
\label{figure:bi-connectivity}
\end{figure}


\begin{enumerate}
\item Vertex $a(x)$ lies on a path in $P_p$

%Consider a vertex $x$ in $T^*$. 
For every vertex $v\in V$ and each path $p_0\in P_p$, we query 
$\cal D$ to compute the edge $(u,v)$ where $u$ is closest 
to $H(p_0)$ on path $p_0$, and add $u$ to $A(v)$. 
%For each path $p_0\in P_p$ we  query 
%$\cal D$ for an edge $(u,x)$ such that the endpoint $u$ is closest 
%to $H(p_0)$ on path $p_0$, and add $u$ to $A(x)$. 
Note that if $a(x)$ lies on $p_0$, for $v=x$ the computed vertex 
$u$ will be same as $a(x)$. %Thus this takes care of the case when
%$a(x)$ belongs to a path in $P_p$.

\item Vertex $x$ lies on a path in $P_p$

For each $u\in T^*$ and $p_0\in P_p$, we query $\cal D$ for an edge
$(u,y)$ such that the 
endpoint $y$ is farthest from $H(p_0)$ on path $p_0$. We add $u$ to $A(y)$. 
Now, consider a vertex $x$ on $p_0$ such that $a(x)=u$. If $x$ is equal to
$y$, then we have added $a(x)$ (i.e. $u$) to $A(x)$. If $x$ is not equal to
$y$, then we have added $a(x)$ (i.e. $u$) to $A(y)$ where $y$ is descendant 
of $x$ in $T^*$. 

\item Vertex $x$ and $a(x)$ lies on same path in $P_t$

For every vertex $v\in p_0$ for a path $p_0\in P_t$, 
we query $\cal D$ to compute the edge $(u,v)$ where $u$ is closest 
to $H(p_0)$ on path $p_0$, and add $u$ to $A(v)$. 
%Consider a vertex $x$ lying on path $p_0\in P_t$. We query $\cal D$ 
%for an edge $(u,x)$ such that the endpoint $u$ is closest to $H(p_0)$ on path 
%$p_0$, and add $u$ to $A(x)$. 
Note that for $x=v$, if $a(x)$ also lies on $p_0$, then $u$  
will be same as $a(x)$. %Thus this takes care of the case when $x$ and $a(x)$
%belongs to same path in $P_t$.



\item Vertex $x$ and $a(x)$ lies on different paths in $P_t$

% For each vertex $x$ belonging to a tree $T_0$ in $\TT$, we calculate
% the highest ancestor of $z$ of $x$ in $T_0$ which has an edge incident 
% from $T_0$. (This is done before the beginning of the algorithm). Now once
% $T^*$ is constructed let $p_z$ be the path in $P_t$ in which vertex $z$
% lies. We query $\cal D$ for an edge $(u,x)$ such that the end 
% point $u$ is closest to $H(p_z)$ on path $p_z$, and add $u$ to $A(x)$. 
% We would show that if (i) $a(x)$ lies in $T_0$, (ii) $x$ and $a(x)$ belongs to
% different paths in $P_t$, and (iii) $(x,a(x))$ is not a newly added edge,
% then $u$ must be same as $a(x)$. 
% 
% We first note that $x$ and $a(x)$ would belong to same tree only (i.e. $T_0$)
% since by our tree partitioning we have that an edge which was earlier present 
% in $G$ cannot have its endpoint in different trees in $\TT$. In order to show
% $u=a(x)$ it is sufficient to prove that $a(x)$ must lie on path $p_z$. Recall that
% our partitioning $\PP\cup \TT$ changes as the algorithm proceeds.
% Let $T_1$ be the tree in $\TT$ containing vertex $z$ just before $p_z$ is 
% attached to $T^*$. Then $T_1$ must be either equal to $T_0$, or a subtree
% of $T_0$. (See Figure \ref{figure:bi-connectivity}). Also $a(x)$ must lie in
% tree $T_1$, since it cannot be an ancestor of $z$ in $T_0$. Now let $T_2$ be
% the tree containing $x$ which is obtained on removal of $p_z$ from $T_1$.
% Note that vertices in $T_2$ must be hanging either from vertex $z$ or some
% descendant of $z$ in $T^*$. Thus the highest ancestor in $T^*\cap V(T_0)$
% which has an edge incident from $x$ must lie on path $p_z$. 

Let $x$ belong to $T_0$ in the initial disjoint tree partitioning $\TT\cup\PP$.
We claim that $a(x)$ would also belong to same tree $T_0$. 
This is because disjoint tree partitioning ensures the absence of edges between two subtrees in $\TT$. 
%We first note that $x$ and $a(x)$ would belong to same tree (say $T_0$) in $\TT$, % only (say $T_0$)
%since disjoint tree partitioning ensures the absence of edges between two subtrees in $\TT$. % does not share edge originally present in $G$
%%since by our tree partitioning we have that an edge originally present in $G$
%%cannot have its endpoint in different trees in $\TT$. 
Let $z$ be the highest ancestor of $x$ in $T_0$ such that $(x,z)$ is an edge in $G+U$. 
Let $p_z$ be the path in $P_t$ containing vertex $z$. 

We now prove that $a(x)$ belongs to $p_z$. Recall that as the algorithm 
%We first show that $a(x)$ must belong to $p_z$. Recall that as the algorithm 
proceeds, our partitioning $\PP\cup \TT$ evolves with time.
Let $T_1$ be the tree in $\TT$ containing vertex $z$ just before $p_z$ is attached to $T^*$. 
%Then $T_1$ must be either equal to $T_0$, or a subtree of $T_0$. (See Figure \ref{figure:bi-connectivity}). 
Then $T_1$ is either same as $T_0$, or a subtree of $T_0$ (see Figure \ref{figure:bi-connectivity} (i)). 
Also, $a(x)$ must lie in tree $T_1$ since it cannot be an ancestor of $z$ in $T_0$. 
Now, let $T_2$ be the tree containing $x$ which is obtained on removal of $p_z$ from $T_1$.
Since $z$ is an ancestor of $x$ in $T_0$, the vertices in $T_2$ will eventually hang from some descendant of $z$ (not necessarily proper) in $T^*$.
For $a(x)$ to be the highest neighbor of $x$ in $T^*$, it should be an ancestor of $z$ in $T^*$, which is only possible if $a(x)\in p_z$.
%Note that vertices in $T_2$ must be hanging either from vertex $z$ or some
%descendant of $z$ in $T^*$. Hence $a(x)$ must belong to $p_z$. 

Therefore, for each vertex $x$ belonging to a tree $T_0$ in $\TT$, we calculate
the highest ancestor $z$ of $x$ in $T_0$ such that $(x,z)$ is an edge in $G+U$.
%which has an edge incident from $T_0$. 
We compute a list $l(z)$ that consist of all the vertices $x$ whose highest ancestor in $T_0$ is $z$.
Now, when $p_z$ is added to $T^*$, we process $l(z)$ as follows.
%Now, once $T^*$ is constructed let $p_z(\in P_t)$ be the path containing
%vertex $z$. 
For every $v\in l(z)$, we query $\cal D$ for an edge $(u,v)$ 
where $u$ is closest to $H(p_z)$ on path 
%such that the endpoint $u$ is closest to $H(p_z)$ on path 
$p_z$, and add $u$ to $A(v)$. Note that if $a(x)$ also lies in $T_0$, then $u$  
must be same as $a(x)$ (see Figure \ref{figure:bi-connectivity} (iii)). 
%This completes our last case.



\end{enumerate}

Now, in the first two steps the total time taken is dominated by the number of 
queries between each path in $P_p$ and the vertices in $T$, i.e., $|P_p|\times n\times \log^3 n=O(nk\log^4n)$.
In the last two steps the total time taken is dominated by a single query for each vertex in $T$,
i.e., $n\times \log^3 n=O(n\log^3 n)$.
Thus, we have the following theorem.

%Note that the total time taken by the first two steps is bounded by
%$O(nk\log^4 n)$ and by the last two steps is bounded by $O(n\log^3 n)$.
%Thus, we have the following theorem.

\begin{theorem}
Given an undirected graph $G(V,E)$ with $|V|=n$ and $|E|=m$, we can maintain a
data structure for answering queries of biconnected components and 2 edge connectivity 
in a dynamic graph which takes $O(\sqrt{mn} \log^{2.5} n)$ update time, $O(1)$ query 
time and $O(m\log n)$ time for preprocessing.
\end{theorem}



==> New folder/conclusion.tex <==
%\section{Applications}
%\label{sec:apnIntro}
%Our fully dynamic algorithm for maintaining a DFS tree can  be used to solve 
%various dynamic graph problems such as dynamic subgraph connectivity, bi-connectivity and 2 edge connectivity.
%Note that these problems are solved trivially using DFS tree in the static setting.
%The solution of dynamic subgraph connectivity follows seamlessly from our fully dynamic algorithm as follows.
%As mentioned in Section \ref{sec:prelim}, we maintain a DFS tree rooted at a dummy vertex $r$, such that
%the subtrees hanging from its children corresponds to connected components of the graph. 
% %we maintain a dummy vertex $r$ as the root of the DFS tree.
%%The DFS tree for each component is a child subtree of $r$. 
%Hence the connectivity query for any two vertices 
%can be answered by comparing their ancestors at depth two (i.e. children of $r$).
%This information can be stored for each vertex and updated whenever the DFS tree is updated.
%Thus we have a data structure for subgraph connectivity with worst case $\tilde{O}(\sqrt{mn})$ update time 
%and $O(1)$ query time. Similarly our algorithm can be used to solve dynamic subgraph bi-connectivity and  
%2-edge connectivity in the same time bounds. For details refer to Appendix \ref{sec:appn}.

\section{Conclusion}
\label{sec:Conclusion}
We have presented a fully dynamic algorithm for maintaining a DFS tree that takes worst case $\tilde{O}(\sqrt{mn})$ update time.
This is the first fully dynamic algorithm that achieves $o(m)$ update time.
% in any dynamic setting.
In the fault tolerant setting our algorithm takes $\tilde{O}(nk)$ time to report a DFS tree, where $k$ is the number of 
vertex or edge failures in the graph. %updates on the graph. 
%In the fully dynamic setting our algorithm takes 
%worst case $\tilde{O}(\sqrt{mn})$ time per update. 
We show the immediate applications of 
fully dynamic DFS for solving various problems such as dynamic subgraph connectivity, biconnectivity and 2-edge connectivity.
We also prove the conditional lower bound of $\Omega(n)$ on maintaining DFS tree under vertex/edge updates.
%Refer to \ref{sec:LowerBounds} for details.




	DFS tree has been extensively used for solving various graph problems in the static setting. 
Most of these problems are also solved efficiently in the dynamic environment.
However, their solutions have not used dynamic DFS tree. 
Furthermore, solutions to most dynamic graph problems under edge updates requires $o(n)$ update time.
However, this is not true for the vertex update variants of these problems.
In the light of $\Omega(n)$ lower bound for updating DFS under both edge and vertex updates, it becomes clear 
that dynamic DFS tree would be more applicable in dynamic graph problems under vertex updates.
The applications of our fully dynamic algorithm follows from the fact that it handles vertex updates 
which was not the case with the existing algorithms for maintaining DFS tree in any dynamic setting. 
% which would have been 
%a natural choice considering 
%their solution using DFS tree in the static setting. 
This paper is thus an attempt to restore the glory of DFS trees for solving graph problems in the dynamic setting 
as was the case in the static setting.
We believe that our dynamic algorithm for DFS, on its own or after further
improvements/modifications, would encourage other researchers to use it in
solving various other dynamic graph problems.







==> New folder/dataStructure2.tex <==
\section{Data Structure}
%\subsection{Data Structure}
\label{sec:data-structure}
The efficiency of our algorithm heavily relies  on the
data structure ${\cal D}$. For any three vertices $w,x,y\in T$, where $path(x,y)$ is an 
ancestor-descendant path in $T$, we need to answer the following two kinds of queries. 
\begin{enumerate}
\item $Query(w,x,y):$ 
among all the edges from $w$ that are incident on $path(x,y)$ %from $w$ 
in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.

\item $Query(T(w),x,y):$ 
among all the edges from $T(w)$ that are incident on $path(x,y)$ %from
in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.
\end{enumerate}

%We now describe this in detail. 
We now describe construction of the data structure $\cal D$. It employs
%Its construction employs 
a combination of two well known techniques, 
namely, heavy-light decomposition \cite{SleatorT83} and suitable augmentation of a binary tree (segment tree)
as follows. 
%Similar techniques were also used for the orthogonal range searching problem \cite{Lewenstein13}.  
%For a given DFS tree $T$ of the graph $G$, the aim of $\DD$ is to answer the queries described in
%Section \ref{sec:prelim}. To meet this objective data structure $\cal D$ is built as follows:

\begin{enumerate}
\item Perform a preorder traversal of tree $T$ with the following restriction: Upon visiting a vertex $v\in T$, the child
of $v$ that is visited first is the one storing the largest subtree. 
Let ${\cal L}$ be the list of vertices ordered by this traversal.
\item Build a segment tree $\TB$ whose leaf nodes from left 
to right represent the vertices in list ${\cal L}$.
\item Augment each node $z$ of $\TB$ with a binary search tree ${\cal E}(z)$, storing all the edges $(u,v)\in E$ where
$u$ is a leaf node in the subtree rooted at $z$ in $\TB$. These edges are sorted according to the position of the second endpoint in ${\cal L}$.
%
%BST ${\cal E}(z)$ containing all the edges $(u,v)\in E$ where
%$u$ is a leaf node in the subtree rooted at $z$ in $\TB$. These edges are ordered by position of $v$ in ${\cal L}$.  
\end{enumerate}


\begin{figure}[ht]
\centering
\includegraphics[width=.9\linewidth]{Figures/DS3.pdf}
\caption{(i) The highest edge from subtree $T(w)$ on $path(x,y)$ is edge $(x,s)$ 
and the lowest edges are edge $(z,w)$ and $(z,t)$.
(ii) The vertices of $T(w)$ are represented as union of two subtrees in segment tree $\TB$.}
\label{fig_xfast}
\end{figure}



The construction of $\DD$ described above ensures the following properties which are helpful in answering a query $Query(T(w),x,y)$ (see Figure \ref{fig_xfast}).
\begin{itemize}
\item $T(w)$ is present as an interval of vertices in $\cal L$ (by step 1). 
Moreover, this interval can be expressed as a union of $O(\log n)$ disjoint subtrees in $\TB$ (by step 2).
Let these subtrees be ${\TB}(z_1),\ldots,{\TB}(z_q)$.
\item It follows from the heavy-light decomposition used in step 1 that path $path(x,y)$ can be divided into $O(\log n)$ subpaths
 $path(x_1,y_1),\ldots,path(x_\ell,y_\ell)$ such that each subpath $path(x_i,y_i)$ is an interval in $\cal L$. %Let these subpaths be 
%\item Any interval of $\cal L$ corresponding to $T(w)$ can be represented by a union of $O(\log n)$ disjoint subtrees $T_j$
%in $\TB$ (by step 2).
\item %Let $z_j$ be the root of subtree ${\cal T}_j$ in $\TB$. 
Let query $Q(z,x,y)$ return the edge on $path(x,y)$ from the vertices in the subtree $\TB(z)$,  
that is closest to vertex $x$. %to query on BST ${\cal E}(z_j)$
Then it follows from step 3 that any query $Q(z_j,x_i,y_i)$ can be answered by a single predecessor or successor query on BST ${\cal E}(z_j)$ in $O(\log n)$ time.
%a path appearing as an interval in $\cal L$, and $T'$ be a subtree of $T$ whose vertices correspond to the leaves
%of a subtree of $\TB$ rooted at some vertex $z$.  
\end{itemize}

%Let $T(w)$ and $path(x,y)$ respectively be any arbitrary subtree and path in $T$. Exploiting the properties of $\DD$ mentioned above,
%we can express $T(w)$ as a disjoint union of $O(\log n)$ subtrees $T'_1,\ldots,T_q'$ in $\TB$ and we can express $path(x,y)$ as a disjoint union of
%$O(\log n)$ subpaths $path(x_1,y_1),\ldots,path(x_\ell,y_\ell)$ each subpath appearing as an intervals of $\cal L$.
To answer $Query(T(w),x,y)$, we thus find the edge closest to $x$ among all the edges reported by the queries
$\{ Q(z_j,x_i,y_i) | 1\le j \le q ~\mbox{and}~ 1\le i \le \ell \}$.
%we find the edge closest to $x$ among all the edges reported by 
%$Query(T_j,x_i,y_i)$ where $i\in[1,O(\log n)]$ and $j\in[1,O(\log n)]$. 
%Since in a BST any predecessor or successor query can be answered in $O(\log n)$ time, 
Thus, $Query(T(w),x,y)$ can be answered in $O(\log^3 n)$ time. 
Notice that $Query(w,x,y)$ can be considered as a special case 
where $q=1$ and $\TB(z_1)$ is the leaf node of $\TB$ representing $w$, i.e., $z_1=w$.
%In case of $Query(w,x,y)$, $q=1$ and $T_1$ is the leaf node of $\TB$ representing $w$.
The space required by $\DD$ is $O(m\log n)$ as each edge is stored at $O(\log n)$ levels in $\TB$. 
Now, the segment tree $\TB$ can be built in linear time. Further, for every node $u\in \TB$, the sorted list of edges 
in ${\cal E}(u)$ can be computed in linear time by merging the sorted lists of its children. 
Thus, the binary search tree ${\cal E}(u)$ for each node $u\in \TB$ can be built in time
linear in the number of edges in ${\cal E}(u)$.
%Further both segment tree and binary search tree can be built in linear time. 
Hence the total time required to build this data structure is $O(m\log n)$. 
Thus, we have the following theorem.

\begin{theorem}
The queries $Query(T(w),x,y)$, $Query(w,x,y)$ on $T$ can be answered in $O(\log^3 n)$ 
worst case time using a data structure $\DD$ of size $O(m \log n)$, which  
can be built in $O(m\log n)$ time.
\label{thm:DS}
\end{theorem}

\noindent \textbf{Note: } 
Procedure~\ref{alg:re-root} can also use a simpler version of $\cal D$ 
which requires a smaller query time. However, our \textit{generic} algorithm 
(described in Section~\ref{sec:algo}) would require these additional features of $\cal D$ 
as follows.
\begin{enumerate}
\item For Procedure~\ref{alg:re-root}, the binary search tree ${\cal E}(u)$ stored at each node $u$
of $\TB$ can be 
replaced by an array storing the sorted list of edges, making it simpler to implement. 
However, our \textit{generic} algorithm also requires deletion of edges from $\DD$. An edge %$(u,v)$ 
can be deleted from $\cal D$ by deleting the edge from the binary search trees
stored at its endpoints %($u$ and $v$) 
and their ancestors in $\TB$. Since a deletion in a binary search tree takes $O(\log n)$ time, 
an edge can be deleted from $\DD$ in $O(\log^2 n)$ time.
\item Procedure~\ref{alg:re-root} only performs the second type of query, i.e., $Query(T(w),x,y)$.
Thus, it would essentially be querying only the part of $path(x,y)$ comprising of the ancestors of $w$ in 
$path(x,y)$. This is thus equivalent to $Query(T(w), LCA(x,w),$ $LCA(y,w))$ (see Figure~\ref{fig_xfast}), 
which will answer the required query as the only edges from $T(w)$ in this interval are incident on $path(x,y)$. 
In such a case, heavy-light decomposition and hence division of $path(x,y)$ to $O(\log n)$ subpaths would not be required. 
Hence, on each node in $u\in\TB$, the query is performed for a single path, requiring total $O(\log^2 n)$ time. 
However, our \textit{generic} algorithm also uses the first type of query, i.e.,  $Query(w,x,y)$, 
where $w$ can be an ancestor of $x$ and $y$. In such a case, we need to perform the query 
only on contiguous intervals of ${\cal L}$ as the interval between $x$ and $y$ in $\cal L$ 
would have several other edges from $w$ that are not incident on $path(x,y)$. 
This necessitates the use of heavy-light decomposition and hence each query requires $O(\log^3 n)$
time.
\end{enumerate} 




%Our algorithm also requires deletion of edges from $\DD$. An edge %$(u,v)$ 
%can be deleted from $\cal D$ by deleting the edge from the binary search tree
%stored at its end points %($u$ and $v$) 
%and their ancestors in $\TB$. 
%Since a deletion in binary search tree takes $O(\log n)$ time, an edge can be deleted from $\DD$ in $O(\log^2 n)$ time.

%\noindent \textbf{Note: } The above data structure could also be made by keeping a 
%sorted array instead of BST at each node of $\TB$. We keep a BST to allow deletion 
%of edges as required in our algorithm. An edge can be deleted from $\cal D$ in 
%$O(\log^2 n)$ time, for deleting the edge from BST of each end node and its 
%ancestors. 


%For any three vertices $w,x,y\in T$, where $path(x,y)$ is an 
%ancestor-descendant path in $T$ we need to answer two kinds of queries. 
%\begin{enumerate}
%\item $Query(w,x,y):$ 
%among all the edges from $w$ that are incident on $path(x,y)$ %from $w$ 
%in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.
%
%\item $Query(T(w),x,y):$ 
%among all the edges from $T(w)$ that are incident on $path(x,y)$ %from
%in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.
%\end{enumerate}


%We perform a 
%%special DFS 
%preorder traversal of the tree $T$ such that from each vertex 
%we first traverse the child with largest subtree rooted at it.
%%of a vertex in the decreasing order of the size of the subtrees hanging from them. 
%Let ${\cal L}$ be the list of the vertices of $T$ 
%arranged in the order of their visit time during this traversal.
%%For notational convenience henceforth, a vertex will also be denoted by its
%%visit-number. Thus ${\cal L}[i]$ is equal to vertex $i$. Also ${\cal L}[i,j]$ 
%%denotes the sequence of vertices from $i$ to $j$. 
%This preorder traversal ensures that any subtree of $T$ is represented by
%a contiguous sequence of vertices in $\cal L$. 
%Further it ensures that 
%any path in $T$ can be partitioned into $O(\log n)$ paths in $T$
%such that each of these paths is a contiguous sequence of vertices in $\cal L$. 
%%vertices (i.e. vertices having contiguous visit times). 
%This property was 
%earlier used in heavy-light decomposition by Sleator and Tarjan 
%\cite{SleatorT83} for dynamic trees. 
%Consider a path $path(x,y)$.
%Let $path(x_1,y_1),...,path(x_k,y_k)$ be the partition of $path(x,y)$ into $k$ paths 
%as described above.% that constitute $path(x,y)$, where $k=O(\log n)$.
%The query $Query(T(w),x,y)$ can thus be answered by finding the edge closest to $x$ among 
%the edges reported by the queries $Query(T(w),x_1,y_1),...,$ $Query(T(w),x_k,y_k)$.


%\begin{figure*}[!ht]
%\centering
%\includegraphics[width=\linewidth]{Figures/DS2.pdf}
%\caption{(i) The highest edge from subtree $T(w)$ on $path(x,y)$ is edge $(x,s)$ 
%and the lowest edges are edge $(z,w)$ and $(z,t)$.
%(ii) The vertices of $T(w)$ are represented as union of two subtrees in segment tree $\TB$.}
%\label{fig_xfast}
%\end{figure*}



%We now describe an efficient data structure to answer the query $Query(T(w),x_i,y_i)$ where
%both $T(w)$ and $path(x_i,y_i)$ are contiguous sequences of vertices in $\cal L$.
%Let $\TB$ be a segment tree \cite{Bentley77} whose leaf nodes from left 
%to right represent the vertices in list ${\cal L}$ (see Figure \ref{fig_xfast}).
%We know that any interval of leaves of $\TB$ can be represented by union of
%$O(\log n)$ disjoint subtrees in $\TB$. Let $T_1,...,T_\ell$ be the subtrees in $\TB$ 
%that covers exactly the leaves of $\TB$ corresponding to $T(w)$ as described above,
% where $\ell=O(\log n)$.
%The query $Query(T(w),x_i,y_i)$ can thus be answered by finding the edge closest to $x_i$ among 
%the edges reported by $Query(T_1,x_i,y_i),...,Query(T_\ell,x_i,y_i)$. Note that for
%$Query(w,x_i,y_i)$, $\ell=1$ as query on only the leaf node in $\TB$ corresponding to $w$ is required.


%Consider an edge $(u,v)$ in $G$. 
%Both $u$ and $v$ are leaf nodes in $\TB$ and have $O(\log n)$ ancestors each. 
%We store the edge as the ordered pair
%$(u,v)$ at all ancestors of $v$ (including itself) in tree $\TB$. 
%Similarly we store the edge as the ordered pair $(v,u)$ at all the ancestors of $u$ 
%(including itself) in tree $\TB$. Thus each edge in $G$
%is stored at $O(\log n)$ levels in $\TB$. Let ${\cal E}(b)$ be the collection of edges 
%stored at any node $b$ in $\TB$. 
%We keep the sets ${\cal E}$ of edges sorted in a balanced binary search tree where each vertex
%is ordered by its position in the list $\cal L$. Thus the query $Query(T_j,x_i,y_i)$ can be answered
%using a single predecessor or successor query on root of $T_j$ as follows. If $x_i$ occurs before 
%$y_i$ in $\cal L$ (or $x_i$ is an ancestor of $y_i$ in $T$) we report the edge $(x,z)$ for some
%vertex $z$ or its successor. Else if $x_i$ occurs after $y_i$ in $\cal L$ (or $x_i$ is a descendant %of $y_i$ in $T$) we report the edge $(x,z)$ for some vertex $z$ or its predecessor.


%Since in a binary search tree any predecessor or successor query can be answered in 
%$O(\log n)$ time, a query $Query(T(w),x,y)$ can be answered in $O(\log^3 n)$ time 
%by finding the edge closest to $x$ among the edges reported by $Query(T_j,x_i,y_i)$ where $i\in[1,k]$ %and $j\in[1,\ell]$. 
%The space complexity is $O(m\log n)$ as each edge is stored at $O(\log n)$ levels. 
%Further both segment tree and binary search tree can be built in linear time. 
%Hence the total time required to create $\TB$ and a binary search tree on ${\cal E}(b)$ for 
%each node $b$ in $\TB$ is $O(m\log n)$. Hence we have the following theorem.

%\begin{theorem}
%The queries $Query(T(w),x,y)$, $Query(w,x,y)$ on $T$ can be answered in $O(\log^3 n)$ 
%worst case time by using $O(m \log n)$ space data structure $\DD$. 
%The time for the construction of the data structure is $O(m\log n)$.
%\label{thm:DS}
%\end{theorem}

%Also to support deletion of edges from the data structure $\cal D$ we have the following
%\begin{lemma}
%Let $E_D$ be a set of edges in $G$ of size $O(k)$. Then the edges $E_D$ can be deleted 
%from the data structure $\DD$ in time $O(k\log^2 n)$ time.
%\label{lem:Del_DS}
%\end{lemma}
%\begin{proof}
%Each edges $e\in E_D$ is stored in $O(\log n)$ binary search trees corresponding to
%${\cal E}$ of $O(\log n)$ nodes of $\TB$. Deleting an edge from a binary search tree
%takes $O(\log n)$ time. Note that these binary search trees may end up skewed after
%these deletions, however the height of each tree will still be bounded by $O(\log n)$.
%Hence, the total time required is $O(\log^2 n)$ time per edge deletion.
%\end{proof}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%   OLD VERSION  %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%











\begin{comment}
\subsection{Data Structure}
\label{sec:data-structure}
The efficiency of our dynamic algorithm relies heavily on the
data structure ${\cal D}$.% We now describe it in detail. 
Its construction employs a combination of two well known techniques, 
namely, heavy-light decomposition and suitably augmented segment tree. 
Similar combination of techniques was also used for the orthogonal 
range searching problem \cite{Lewenstein13}.  

For any three vertices $w,x,y\in T$, where $path(x,y)$ is an 
ancestor-descendant path in $T$ we need to answer two kinds of queries. 
\begin{enumerate}
\item $Query(w,x,y):$ 
among all the edges from $w$ that are incident on $path(x,y)$ %from $w$ 
in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.

\item $Query(T(w),x,y):$ 
among all the edges from $T(w)$ that are incident on $path(x,y)$ %from
in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.
\end{enumerate}

We perform a 
%special DFS 
preorder traversal of the tree $T$ such that from each vertex 
we first traverse the child with largest subtree rooted at it.
%of a vertex in the decreasing order of the size of the subtrees hanging from them. 
Let ${\cal L}$ be the list of the vertices of $T$ 
arranged in the order of their visit time during this traversal.
For notational convenience henceforth, a vertex will also be denoted by its
visit-number. Thus ${\cal L}[i]$ is equal to vertex $i$. Also ${\cal L}[i,j]$ 
denotes the 
sequence of vertices from $i$ to $j$. This preorder %special DFS 
traversal ensures that 
any path in $T$ can be represented by $O(\log n)$ contiguous sequences of 
vertices (i.e. vertices having contiguous visit times). This property was 
earlier used in heavy-light decomposition by Sleator and Tarjan 
\cite{SleatorT83} for dynamic trees. 

In order to answer the queries on $T$, we define two additional queries on 
list ${\cal L}$. Let $i,j,p,q$ be integers in the range $1$ to $n$ satisfying
the relation $i\leq j<p\leq q$. The two queries on ${\cal L}$ are -


\begin{itemize}
\item $Q_F(i,j,p,q):$ Reports an edge $(a,b)$ s.t. $a$ is the first vertex in 
list ${\cal L}[i,j]$ having an edge incident on it from some $b$ in 
${\cal L}[p,q]$.
\item $Q_L(i,j,p,q):$ Reports an edge $(a,b)$ s.t. $a$ is the last vertex in
list ${\cal L}[i,j]$ having an edge incident on it from some $b$ in ${\cal L}[p,q]$.
\end{itemize} 

%########

%For notational convenience we use $Q$ when we are referring to both $Q_F$ and $Q_L$.
%Hence the query $Query(T(w),x,y)$ or $Query(w,x,y)$ is from a contiguous sequence of vertices
%in $\cal L$ (representing the tree $T(w)$ or $w$) to the path $path(x,y)$ in $T$.
%This 
%from subtree or a vertex to 

\begin{lemma}
The two queries, $Query(T(w),x,y)$ and $Query(w,x,y)$, on the DFS tree $T$ 
can be answered using at most $O(\log n)$ queries of $Q_F$ and $Q_L$ on list 
${\cal L}$.
\label{lem:equivalence}
\end{lemma}

\begin{proof}
Consider the query $Query(T(w),x,y)$ on tree $T$. Let $p$ and $q$ be the visit time
of first and last visited vertices in the subtree $T(w)$. Then ${\cal L}[p,q]$ is the 
contiguous sequence corresponding to the vertices in subtree $T(w)$ (see Figure 
\ref{fig_xfast}). For each vertex $w$, we can precompute these two numbers $p$ and $q$ 
during preprocessing.
Note that in case of $Query(w,x,y)$, the values of $p$ and $q$ are the same representing $w$ in $T$.
 Let $path(x_1,y_1),...,path(x_k,y_k)$ be $k$ contiguous paths 
of $T$ that constitute $path(x,y)$. Note that $k=O(\log n)$ as follows from the 
heavy-light decomposition described above.
The query $Query(T(w),x,y)$ can thus be answered by finding the edge closest to $x$ among 
the edges reported by $Query(T(w),x_1,y_1),...,Query(T(w),x_k,y_k)$.
Further let ${\cal L}[p_i,q_i]$ represent the sequence of vertices of 
$path(x_i,y_i)$ for each $1 \le i \le k$. 
It can be observed that
each query $Query(T(w),x_i,y_i)$ is equivalent to the query $Q_F(p,q,p_i,q_i)$ 
in case $x$ in an ancestor of $y$ and $Q_L(p,q,p_i,q_i)$ otherwise. 
%Similarly $Q(w,x_i,y_i)$ is equivalent to the query $Q_F(p,p,p_i,q_i)$ in case $x$ in 
%an ancestor of $y$ and $Q_L(p,p,p_i,q_i)$ otherwise.
\end{proof}


\begin{figure}[ht]
\centering
\includegraphics[width=.85\linewidth]{Figures/DS.pdf}
\caption{(i) The highest edge from subtree $T(w)$ on $path(x,y)$ is edge $(1,4)$ 
and the lowest edges are edge $(2,3)$ and $(2,5)$.
(ii) The vertices of $T(w)$ are represented as union of two subtrees in segment tree $\TB$.}
\label{fig_xfast}
\end{figure}



We now describe an efficient data structure to answer the queries $Q_F$ and $Q_L$ on
list ${\cal L}$. Let $\TB$ be a segment tree \cite{Bentley77} whose leaf nodes from left 
to right represent the vertices in list ${\cal L}$ (see Figure \ref{fig_xfast}).
We know that any interval $[p,q]$ of leaves of $\TB$ can be represented by union of
$O(\log n)$ disjoint subtrees in $\TB$. Consider an edge $(u,v)$ in $G$. 
Both $u$ and $v$ are leaf nodes in $\TB$ and have $O(\log n)$ ancestors each. 
We store the edge as the ordered pair
$(u,v)$ at all ancestors of $v$ (including itself) in tree $\TB$. 
Similarly we store the edge as the ordered pair $(v,u)$ at all the ancestors of $u$ 
(including itself) in tree $\TB$. Thus each edge in $G$
is stored at $O(\log n)$ levels in $\TB$. Let ${\cal E}(b)$ be the collection of edges 
stored at any node $b$ in $\TB$. 
We keep the sets ${\cal E}$ of edges sorted in the
lexicographic order as a balanced binary search tree.

We now describe how query $Q_F(i,j,p,q)$ is answered by $\TB$ ($Q_L(i,j,p,q)$ can be 
answered in a similar manner):

Let $T_1,...,T_\ell$ be the subtrees in $\TB$ representing the range ${\cal L}[i,j]$.
For each $T_\alpha, 1\le \alpha\le \ell$, we find the predecessor of $(q,n+1)$ 
in the set ${\cal E}(a)$ where $a$ is the root of $T_{\alpha}$. 
This requires a predecessor query on the binary search tree stored at $a$. 
We return the lexicographically largest ordered pair among these edges reported by 
the $\ell$ predecessor queries.

Since in a binary search tree any predecessor or successor query can be answered in 
$O(\log n)$ time, a query $Q_L$ or $Q_F$ can be answered in $O(\log^2 n)$. 
The space complexity is $O(m\log n)$ as each edge is stored at $O(\log n)$ levels. 
Hence the total time required to create $\TB$ and a BST on ${\cal E}(b)$ for 
each node $b$ in $\TB$ is $O(m\log n)$. Hence we have the following lemma.

\begin{lemma}
The queries $Q_F,Q_L$ on list ${\cal L}$ can be answered in $O(\log^2 n)$ worst case
time by using $O(m \log n)$ space data structures. The preprocessing time, i.e. the
time for construction of the data structure is $O(m\log n)$.
\label{lem:DS_time}
\end{lemma}
Using Lemma \ref{lem:equivalence} and Lemma \ref{lem:DS_time} we have the following main
theorem.

\begin{theorem}
The queries $Query(T(w),x,y)$, $Query(w,x,y)$ on $T$ can be answered in $O(\log^3 n)$ 
worst case time by using $O(m \log n)$ space data structure $\DD$. 
The time for the construction of the data structure is $O(m\log n)$.
\label{thm:DS}
\end{theorem}

\begin{lemma}
Let $E_D$ be a set of edges in $G$ of size $O(k)$. Then the edges $E_D$ can be deleted 
from the data structure $\DD$ in time $O(k\log^2 n)$ time.
\label{lem:Del_DS}
\end{lemma}
\begin{proof}
Each edges $e\in E_D$ is stored in $O(\log n)$ binary search trees corresponding to
${\cal E}$ of $O(\log n)$ nodes of $\TB$. Deleting an edge from a binary search tree
takes $O(\log n)$ time. Note that these binary search trees may end up skewed after
these deletions, however the height of each tree will still be bounded by $O(\log n)$.
Hence, the total time required is $O(\log^2 n)$ time per edge deletion.
\end{proof}
\end{comment}


==> New folder/fullyDynamic_4.tex <==
%\section{Fully dynamic DFS}
\section{Fully dynamic DFS}
\label{sec:fullyDyn}
% \begin{lemma}
% Let $P$ be any dynamic graph problem and $G$ be the input graph. 
% Let $f,g,h$ be three functions of $m$,$n$ such that
% there exists a data structure $D$ for $P$ that
% (i) can be preprocessed in $f$ time, and
% (ii) given any set $U$ of $t$ ($t<n$) updates, 
% is able to compute the solution for $G+U$ in $t\times g+h$ time.
% Then, there exists a dynamic algorithm for $P$ with worst case
% $O(\sqrt{fg}+h)$ update time.
% \end{lemma}





We now describe the overlapped periodic rebuilding technique to convert
our algorithm for computing a DFS tree after $k$ updates to fully dynamic 
and incremental algorithms for maintaining a DFS tree. Similar technique was used by 
Thorup \cite{Thorup05} for maintaining fully dynamic all pairs shortest paths. 
 
In the fully dynamic model, we need to report %our algorithm rebuilds 
the DFS tree after every update in the graph. 
Given the data structure $\DD$ built using the DFS tree of the graph $G$, 
we are able to report the DFS tree of $G+U$ after $|U|=k$ updates 
in $\tilde{O}(nk)$ time. This becomes inefficient if $k$ becomes large.
Rebuilding $\DD$ after every update is also inefficient as it takes $\tilde{O}(m)$ time to build $\DD$. 
Thus, it is better to rebuild $\DD$  after every $|U'|=c$ updates for a carefully chosen $c$.
Let $\DD'$ be the data structure built using the DFS tree of the updated graph $G+U'$ with $|U'|=c$.
$\DD'$ can thus be used to process the next $c$ updates efficiently (see Figure \ref{fig:replace} (a)).
The cost of building $\DD'$ can thus be amortized over these $c$ updates. 

To achieve an efficient worst case update time, we divide the building of $\DD'$ 
over the first $c$ updates. This $\DD'$ is then used by our algorithm in the next $c$ updates, during which 
a new $\DD''$ is built in a similar manner and so on (see Figure \ref{fig:replace} (b)). 
The following lemma describes how this technique can 
be used in general for any dynamic graph problem. For notational convenience we denote any function $f(m,n)$ as $f$.

\begin{lemma}
Let $D$ be a data structure that can be used to report the solution of a graph problem after a set of $U$ updates 
on an input graph $G$. If $D$ can be build in $O(f)$ time and the solution for graph $G+U$ can be reported in 
 $O(h+|U|\times g)$ time, then $D$ can be used to report the solution after every update in worst case
$O(\sqrt{fg}+h)$ update time, given that $\sqrt{f/g}\leq n$.%, where $f,g,h$ are functions of $m$ and $n$. 
\end{lemma}



\begin{figure}[ht]
%\begingroup
\centering
\includegraphics[width = \linewidth]{Figures/fullyDynamicfig.pdf}
%\captionof{figure}{
\caption{
(a) Fully dynamic algorithm with amortized update time. %  from the data structure $D$.
(b) De-amortization of the algorithm.}
\label{fig:replace}
%\endgroup
\end{figure}



%\begin{lemma}
%Let $P$ be any graph problem and $G$ be the input graph. 
%Let $D$ be a data structure for $P$ and 
%$f,g,h$ be functions of $m$, $n$ such that
%\begin{itemize}
%\item[(i)] 
%Graph $G$ can be preprocessed to compute $D$ in $O(f(m,n))$ time, and
%\item[(ii)] 
%or any given set $U$ of $k$ ($k<n$) updates, $D$ can be used to 
%compute solution of $P$ for graph $G+U$ in $O(h(m,n)+k\times g(m,n))$ 
%time.
%\item[(iii)] 
%$\sqrt{f(m,n)/g(m,n)}\leq n$,
%\end{itemize}
%Then, there exists a dynamic algorithm for $P$ with worst case
%$O(\sqrt{fg}+h)$ update time.
%\end{lemma}

\begin{proof}
We first present an algorithm that achieves amortized $O(\sqrt{fg}+h)$ 
update time. It is based on the simple idea of periodic rebuilding. Given 
the input graph $G_0$ we preprocess it to compute the data structure $D_0$ over
it. Now, let $u_1,...,u_c$ ($c\leq n$) be the sequence of first $c$ updates 
on $G_0$. To report the solution after $i^{th}$ update we use $D_0$ to compute 
the solution for $G_0+\{u_1,...,u_i\}$. This takes $O(h+(i\times g))$ time. 
So the total time for preprocessing and handling the first $c$ updates is 
$O(f+\sum_{i=1}^c h+(i\times g))$. Therefore, the average time for the first 
$c$ updates is $O(f/c+c\times g+h)$. Minimizing this quantity over $c$ gives
the optimal value $c_0=\sqrt{f/ g}$ which is bounded by $n$. So, after every
$c_0$ updates we rebuild our data structure and use it for the next $c_0$ updates 
(see Figure \ref{fig:replace}(a)). Substituting the value of $c_0$ gives the
amortized time complexity as $O(\sqrt{fg}+h~)$.

The above algorithm can be de-amortized as follows. Let $G_1,G_2,G_3,\ldots$ 
be the sequence of graphs obtained after $c_0,2c_0,3c_0,..$ updates. 
We use the data structure $D_0$ built during preprocessing to handle the first 
$2c_0$ updates. Also, after the first $c_0$ updates we start building the data 
structure $D_1$ over $G_1$. This $D_1$ is built in $c_0$ steps, thus the
extra time spent per update is $f/c_0=O(\sqrt{fg})$ only. 
We use $D_1$ to handle the next $c_0$ updates on graph $G_2$, and also in 
parallel compute the data structure $D_2$ over the graph $G_2$. 
(See Figure \ref{fig:replace}(b)). Since the time for
building each data structure is now divided in $c_0$ steps, we have that the
worst case update time as $O(\sqrt{fg}+h~)$.
\end{proof}



%\begin{figure*}[!ht]
%\centering
%\includegraphics[width = \linewidth]{Figures/fullyDynamicfig.pdf}
%\caption{(a) Obtaining an amortized dynamic algorithm. %  from the data structure $D$.
%(b) Deamortization of the algorithm.}
%\label{fig:replace}
%	\end{figure*}

The above lemma combined with Theorems \ref{main-result} and 
\ref{theorem:insertions-only} directly implies the following results for the 
fully dynamic DFS tree problem and the incremental DFS tree problem, respectively.

%(For the theorem below we use $f=m\log n$, $g=n\log^4 n$ and $h=0$.)
(For the following theorem we use Theorem~\ref{main-result}, implying $f=m\log n$, $g=n\log^4 n$ and $h=0$.)
\begin{theorem}
There exists a fully dynamic algorithm for maintaining a DFS tree in an
undirected graph that uses $O(m\log n)$ preprocessing time and can report a 
DFS tree after each update in the worst case $O(\sqrt{mn} \log^{2.5} n)$ time.
An update in the graph can be insertion / deletion of an edge as well as a
vertex.
\end{theorem}

%(For the theorem below we use $f=m\log n$, $g=\log n$ and $h=n \log^3 n$,
%since $O(n \log^3 n)=O(k\times g+h)$ for $k\leq n$).
(For the following theorem we use Theorem~\ref{theorem:insertions-only}, implying 
$f=m\log n$, $g=\log^3 n$ and $h=n\log^3 n$.)
%since $O(n \log^3 n)=O(k\times g+h)$ for $k\leq n$).
\begin{theorem}
There exists an incremental algorithm for maintaining a DFS tree in an
undirected graph that uses $O(m\log n)$ preprocessing time and can report a 
DFS tree after each edge insertion in the worst case $O(n \log^3 n)$ time.
\end{theorem}



==> New folder/intro.tex <==
\section{Introduction}
Depth First Search (DFS) is a well known graph traversal technique. Right from the seminal work of Tarjan \cite{Tarjan72}, DFS traversal 
has played the central role in the design of efficient algorithms for many fundamental graph problems, namely, biconnected components~\cite{Tarjan72}, 
strongly connected components~\cite{Tarjan72}, topological sorting,
bipartite matching \cite{HopcroftK73}, dominators in directed graph \cite{Tarjan74} and planarity testing \cite{HopcroftT74}.
%Depth First Search (DFS)\index{Depth First Search}\index{DFS}\index{DFS trees} is a well known graph traversal technique. This 
%technique has been reported to be introduced by Charles Pierre Tr\'{e}maux, a 
%19th-century French mathematician who used it for solving mazes. However,
%it was Tarjan, who in his seminal work \cite{Tarjan72}, demonstrated the
%power of DFS traversal for solving various fundamental graph problems, namely,
%topological sorting, connected components, biconnected components and 
%strongly-connected components. Since  then, DFS traversal is one of the most
%widely used graph traversal techniques. 
Interestingly, the role of DFS traversal is not confined to merely the design of efficient algorithms. 
For example, consider the classical result of Erd{\H o}s and R{\' e}nyi \cite{ErdosR60} for the 
phase transition phenomena in random graphs. There exist many proofs of this result which are intricate and based on highly sophisticated probability tools. However, recently, Krivelevich and Sudakov \cite{KrivelevichS13}  designed a truly simple, short, and elegant proof for this result based on the insights from a DFS traversal in a graph.


Let $G=(V,E)$ be an undirected connected graph on $n$ %=|V|$
vertices and $m$ %=|E|$ 
edges. DFS traversal of $G$ starting from any vertex $r\in V$ 
%traverses is a recursive algorithm to traverse a graph. This traversal
produces a rooted spanning tree, %(or forest, in case $G$ is not connected),
called a DFS tree with $r$ as its root. 
It takes $O(m+n)$ time to perform a DFS traversal and generate a DFS tree. 
Given any rooted spanning tree of graph $G$, all non-tree edges of the graph
can be %partitioned 
classified into two categories, namely, back edges and cross edges
as follows. A non-tree edge is called a {\it back edge} if one of its endpoints is an ancestor of the other in the tree. Otherwise, it is called a
{\it cross edge}. A necessary and sufficient condition for any rooted 
spanning tree to be a DFS tree is that every non-tree edge is a back edge.
%So 
Thus, it can be seen that many DFS trees are possible for any given graph. 
However, if the traversal of the graph is performed according to the order specified by the adjacency lists of the graph, the resulting DFS tree will
be unique. The ordered DFS tree problem
is to compute the order in which the vertices get visited when the traversal
is performed strictly according to the adjacency lists.
%Notice that for all algorithmic applications mentioned above, any DFS tree suffices.

Most of the graph applications in real world deal with graphs that keep 
changing with time. These changes/updates can be in the form of insertion 
or deletion of vertices or edges. An algorithmic graph problem is modeled in a dynamic environment as follows. There is an online sequence of 
updates on the graph, and the objective is to update the solution of the problem efficiently after each update. % using some clever data structure.
In particular, the time taken to update the solution has to be much smaller than that of the best static algorithm for the problem. 
In the last two decades, many elegant dynamic algorithms have been designed for various graph problems such as connectivity \cite{EppsteinGIN97,HenzingerK99,HolmLT01,KapronKM13},
reachability \cite{RodittyZ08,Sankowski04},
shortest path \cite{DemetrescuI04,RodittyZ12}, spanners \cite{BaswanaKS12,GottliebR08,Roditty12}, and min-cut \cite{Thorup07}.
Another, and more restricted, variant of a dynamic environment is the fault tolerant environment. Here the aim is to build a compact
data structure for a given problem, that is resilient to failure of vertices/edges, and can efficiently report the 
solution of the problem for any given set of failures. 
There has been a lot of work in the last two decades on fault tolerant algorithms for connectivity 
\cite{ChanPR08,Duan10,FrigioniI00}, shortest paths \cite{BaswanaK13,ChechikLPR12,DemetrescuTCR08}, and spanners
\cite{BraunschvigCPS15,ChechikLPR10}.

A dynamic graph algorithm is said to be \textit{fully dynamic} if it handles both 
insertion as well as deletion updates. A partially dynamic algorithm is said
to be \textit{incremental} or \textit{decremental} if it handles only insertion or only deletion updates respectively. 
%In general hardness of a dynamic graph problem depends on the type 
%of updates it needs to handle. 
%Most of the dynamic graph algorithms consider edge updates only; the vertex %updates are generally much harder to handle as compared to edge updates. 
%Similarly in general, the hardness of a graph problem 
%increases from incremental to decremental to fully dynamic setting. For any %graph 
%problem in general, the worst case upper bounds are much weaker than the %amortized bounds. 
%Similarly deterministic bounds are much weaker than the randomized bounds. %These 
%hardness variations can be seen in the aforementioned results for different %dynamic 
%graph problems. ///relevant citations needed/// 
In this paper, we address the problem of maintaining a DFS tree efficiently in any dynamic environment.  

%-------------------------------------------------------------------------
\subsection{Existing results on dynamic DFS}
%-------------------------------------------------------------------------
In spite of the simplicity of a DFS tree, designing any efficient parallel 
or dynamic algorithm for a DFS tree has turned out to be quite challenging. Reif \cite{Reif85} 
showed that the ordered DFS tree problem is a $P$-Complete problem. 
For many years, this result seemed to imply that the general DFS tree problem,
that is, the computation of any DFS tree, is also inherently sequential. 
However, Aggarwal and Anderson \cite{AggarwalA88} proved that the general
DFS tree problem is in {\em RNC} by designing a parallel randomized algorithm that takes 
$O(\log^3 n)$ expected time. 
Further, the fastest parallel deterministic algorithm for general DFS tree still 
takes $O(\sqrt{n})$ time \cite{AggarwalAK90,GoldbergPV88}.  
Whether the general DFS tree problem is in {\em NC} for directed (or undirected) graphs is still a 
long standing open problem.

Reif \cite{Reif87} and later Miltersen et al. \cite{MiltersenSVT94} proved 
that $P$-Completeness of a problem also implies hardness of the problem in 
the dynamic setting. The work of Miltersen et al. \cite{MiltersenSVT94} 
shows that if the ordered DFS tree is updateable in $O({\mathbf{polylog}}(n))$ time, 
then the solution of every problem in class $P$ is updateable in 
$O({\mathbf{polylog}}(n))$ time. In other words, maintaining the ordered DFS 
tree is indeed the hardest among all the problems in class $P$.
In our view, this hardness result, which is actually for only the ordered
DFS tree problem, has proved to be quite discouraging for the researchers 
working in the area of dynamic algorithms.
This is evident from the fact that for all the static graph problems that
were solved using DFS traversal in the 1970's, none of their dynamic counterparts
used a dynamic DFS tree \cite{HenzingerK99,HolmLT01,KapronKM13,RodittyZ08,Chan06,ChanPR08,Duan10}.

Apart from the hardness of the ordered DFS tree problem in dynamic environment, 
very little progress has been achieved even for the problem
of maintaining any DFS tree. 
Franciosa et al. \cite{FranciosaGN97} designed an incremental algorithm for
a DFS tree in a directed acyclic graph (DAG). % under insertion of edges. 
For any arbitrary sequence of edge insertions, this algorithm takes $O(mn)$ total time to 
maintain a DFS tree from a given source. 
Recently, Baswana and Choudhary \cite{BaswanaC15} designed a decremental algorithm
for a DFS tree in a DAG that requires expected $O(mn\log n)$ total time.
For undirected graphs, recently 
Baswana and Khan \cite{BaswanaK14} designed an incremental algorithm for maintaining a DFS tree
requiring $O(n^2)$ total time. 
These algorithms are the only results known for the dynamic DFS tree problem. 
Moreover, none of these existing algorithms, though designed for only a partially dynamic environment, 
achieves a worst case bound of $o(m)$ on the update time.
% Also despite having an efficient solution for DFS in the incremental setting
%these results did not give any applications implying the usefulness of Dynamic DFS as in case of static DFS.
%
%Note that both these results are for incremental edge updates only and 
%have amortized bounds. Hence the problem remains open for 
%all the harder models of dynamic algorithms as described earlier.
%The importance of handling vertex updates in a DFS tree can even be %highlighted
%by the fact that even a single update may lead to significant change in the %DFS tree in the worst case.
%Hence achieving $O(\polylog n)$ worst case update time seems unlikely, 
%limiting its applications for most dynamic graph problems handling edge %updates.
%However in general dynamic graph problems handling vertex updates often seem %to have harder bounds.
%// CITATIONS NEEDED // 
%Further neither of these algorithms presented its applications to any well studied dynamic graph problems.
%of their algorithm
%improving results for any dynamic graph problems.
Furthermore, none of these results proves that general DFS is not as hard as ordered DFS in the dynamic environment. 
This is because the speculations of having to incur a complete recomputation in the worst case after an update 
is not disproved by amortized bounds resulting in the perceived $O(m)$ {\em barrier} for general DFS as well.  
So the following intriguing questions remained unanswered till date:%\\
\begin{itemize}
%\itemsep-0.5em 
\item
Does there exist any fully dynamic algorithm for maintaining
a DFS tree?
\item 
Is it possible to achieve worst case $o(m)$ update time for maintaining a DFS tree in a dynamic environment?
\end{itemize}

Not only do we answer these open questions affirmatively for undirected graphs, 
we also use our dynamic algorithm for DFS tree to provide efficient 
solutions for a couple of well studied dynamic graph problems. 
%Note that our result is the first use of dynamic DFS for solving dynamic graph problems,
%which was long overdue considering applications of DFS tree in the static setting.
Moreover, our results also handle vertex updates which are generally considered harder than
edge updates.
Furthermore, our results finally prove that general DFS is indeed not as hard as ordered DFS in the dynamic setting
as was the case in parallel setting.
%but we also present the first fault tolerant data structure for a DFS tree. 
%
%----------------------------???????????-------------------------------
% In addition to handle edge updates, our algoritms can handle vertex updates %as well without any extra as edge updates  model which is generally %considered harder than edge update model. 
%
%Moreover, we use our dynamic algorithm for DFS tree for providing very simple and efficient solutions for a couple of well studied dynamic graph problems. 

%-------------------------------------------------------------------------
\subsection{Our results}
%-------------------------------------------------------------------------
%
We consider a generalized notion of updates wherein an update could be either
insertion/deletion of a vertex or insertion/deletion of an edge. For any set
$U$ of such updates, let $G+U$ denote the graph obtained after performing 
the updates $U$ on the graph $G$. Our main result can be succinctly
described in the following theorem.
\begin{theorem} An undirected graph can be preprocessed to build a data 
structure of $O(m \log n)$ size such that for any set $U$ of $k\leq n$ updates, a DFS tree of $G+U$ can be reported in $O(nk \log^4 n)$ 
time.
\label{main-result}
\end{theorem}

With this result at the core, we easily obtain the following %three 
results for dynamic DFS tree in an undirected graph.
\begin{enumerate}
\item {\em Fault Tolerant DFS tree}:

Given any set of $k$ failed vertices or edges, %and any vertex $v\in V$, 
we can report a DFS tree %rooted at $v$ 
for the resulting graph in $O(nk \log^4 n)$ time.
%For the special case of $k=1$, our algorithm takes $O(n \log^3 n)$ time.

%The recent work of Henzinger et al. \cite{HenzingerKNS15} directly implies a 
%conditional lower bound of $\Omega(nk)$ for maintaining a DFS tree 
%(which trivially maintains connectivity information) in a fault tolerant 
%environment after a failure of $k$ vertices. Thus our fault tolerant algorithm
%is optimal upto $O(\polylog~n)$ factors.
%
%--------------???????- We need to write the proof of this in Appendix
%--------------???????- should we say explicit DFS tree--------
%--------------???????- Any lower bound for k failures --------
%

\item {\em Fully Dynamic DFS tree}:

Given any arbitrary online sequence of vertex or edge updates, we can maintain a DFS tree in $O(\sqrt{mn} \log^{2.5} n)$ worst case time per update. 
%For graphs with $m=\Theta(n^2)$ edges, this algorithm achieves 
%an improvement by a factor of $\sqrt{n}$ over the static algorithm.

%A simple reduction from recent work of Abboud and Williams \cite{AbboudW14} implies a
%conditional lower bound of $\tilde{\Omega}(n)$ \footnote{where $\tilde{()}$ denotes ignoring $%\polylog~n$ factors} amortized update time for maintaining a fully dynamic DFS tree 
%under vertex updates.
%We also present an unconditional lower bounds of $\tilde{\Omega}(n)$ for maintaining a fully dynamic %DFS tree under edge updates if the DFS tree is maintained explicitly.

\item {\em Incremental DFS tree}:

Given any arbitrary online sequence of edge insertions, we can maintain
a DFS tree in $O(n \log^{3} n)$ worst case time per edge insertion. 

%The reduction from recent work of Abboud and Williams \cite{AbboudW14} also implies a
%conditional lower bound of $\omega(n^{1-\epsilon})$ (for any $\epsilon<1$) worst case update time for maintaining an incremental or decremental DFS tree 
%under vertex updates.
%Note that our incremental algorithm for edge updates matches the lower bound for the same problem %under vertex updates.

\end{enumerate} 

These are the first $o(m)$ worst case update time algorithms for maintaining a DFS tree in a dynamic environment. 
%
%\noindent
%{\em Remark}:
Recently, there has been significant work
%There has been recent work 
\cite{AbboudW14, HenzingerKNS15} on establishing conditional lower bounds on the time complexity of various dynamic graph problems.
A simple reduction from [1], based on the Strong Exponential Time Hypothesis (SETH), implies a conditional lower bound of  ${\Omega}(n)$ on the update time of any fully dynamic algorithm for a DFS tree under vertex updates. 
%This matches the upper bound of our Fault
%tolerant algorithm (upto polylog factors) if the number of failures is O~(1).
%--------Objection:
%--------Fault tolerant is a weaker version of fully dynamic encironmnet.
%--------So if you have a proof for the fault tolerant, then
%--------we may write the following statement:
%-------- 
We also present an unconditional lower bound of $\Omega(n)$ for
maintaining a fully dynamic DFS tree explicitly under edge updates.
%For more details refer to the full version of the paper.% (refer to full paper for details).
% if the DFS tree has to be maintained {\em explicitly}.


%\item{\em rerooting a DFS tree}
%Given any DFS tree $T$, it takes $O(n\log^3 n)$ time to reroot $T$ at any %arbitrary vertex in the graph. Interestingly, there was no non-trivial
%algorithm for rerooting a DFS tree in the past. 


%\noindent
%These are the first $o(m)$ update time algorithms for the maintaining a 
%DFS tree in a dynamic setting. 
%These upper bounds gets more significant in the light of the lower bounds.
%We also present conditional lower bounds of $\Omega(n)$ on the update 
%time for maintaining DFS tree in a fully dynamic environment. Therefore, 
%our results are off from optimal by a factor of $\tilde{O}(k)$ for the 
%fault tolerant setting and by a factor of $\tilde{O}(\sqrt{m/n})$ for the 
%fully dynamic maintenance of DFS tree. 
%We now demonstrate the applications of our fully dynamic DFS tree algorithm

\subsection{Applications of Fully Dynamic DFS}

In the static setting, a DFS tree can be easily used to answer connectivity, 2-edge connectivity and biconnectivity queries.
Our fully dynamic algorithm for DFS tree thus seamlessly solves these problems for both vertex and edge updates.
Further, our result gives the first deterministic algorithm with $O(1)$ query time and $o(m)$ worst case update time 
for several well studied variants of these problems in the dynamic setting.
These problems include dynamic subgraph connectivity \cite{ChanPR08,Duan10,EppsteinGIN97,Frederickson85,HolmLT01,KapronKM13} 
and vertex update versions of dynamic biconnectivity \cite{Henzinger00,Henzinger95,HolmLT01} and dynamic 2-edge connectivity \cite{HolmLT01,EppsteinGIN97,Frederickson85}. 
The existing results offer different trade-offs between the update time and the query time, and differ on the types 
(amortized or worst case) of update time and the types (deterministic or randomized) of query time. 
Our algorithm, in particular, improves the deterministic worst 
case bounds for these problems, thus demonstrating %emphasizing %implying 
the relevance of
DFS trees in solving dynamic graph problems.% (refer to full paper for details).




%%%%Earlier Version:
%Our fully dynamic algorithm for a DFS tree provides a new, simple, and efficient algorithm 
%for the dynamic subgraph connectivity problem.
%This problem, first introduced by Frigioni and Italiano \cite{FrigioniI00} for planar graphs, can be described as follows.
%There is an undirected graph where the status of each vertex is either
%{\it active} or {\it inactive} at a time. An update involves switching the
%status of any vertex from active to inactive, or vice versa. The goal is to maintain a compact data structure that can efficiently answer connectivity query between any two vertices on the subgraph induced by the active vertices.
% 
%There exists many efficient algorithms for the dynamic subgraph connectivity
%\cite{ChanPR08,Duan10,EppsteinGIN97,Frederickson85,HolmLT01,KapronKM13}. These algorithms offer different trade-offs between the update time and the query time, and differ on the types (amortized or worst case) of update time and
%the types (deterministic or randomized) of query time. 
%The previous deterministic results for this problem that achieve $o(m)$ worst case update time are as follows. Duan \cite{Duan10} achieves $\tilde{O}(m^{4/5})$ update time and $O(m^{1/5})$ query time, and Eppstein et al. \cite{EppsteinGIN97} achieve $O(n\sqrt{n})$ update time and $O(1)$ query time. 
%We, as a direct application of our fully dynamic DFS tree algorithm, can achieve $\tilde{O}(\sqrt{mn})$ worst case update time and $O(1)$ query time 
%for the dynamic subgraph connectivity. 
%Moreover, our algorithm extends to dynamic subgraph bi-connectivity and dynamic subgraph 2-edge connectivity in a straightforward manner.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Our fully dynamic DFS tree provides a new, simple, and efficient algorithm 
%for the dynamic subgraph connectivity problem which can be described as follows.
%% in the context of planar graphs. %For any
%%general graph, the problem can be described as follows.
%Given an undirected graph where the status of each vertex can be switched between 
%{\it active} and {\it inactive} in an update. 
%The goal is to maintain a compact data structure that can efficiently answer 
%connectivity query between any two vertices in the subgraph induced by the active vertices. 
%Note that this is a weaker model as compared to fully dynamic connectivity under vertex updates.
%Thus any algorithm for fully dynamic connectivity under edge updates trivially solves dynamic subgraph connectivity
%at the expense of $O(n)$ factor in update time. 
%This is because switching a vertex active or inactive is equivalent to $O(n)$ edge updates. 

%Our fully dynamic algorithm for a DFS tree provides a new, simple, and efficient algorithm 
%for the dynamic subgraph connectivity problem.
%This problem, first introduced by Frigioni and Italiano \cite{FrigioniI00} for planar graphs, can be described as follows.
%% in the context of planar graphs. %For any
%%general graph, the problem can be described as follows.
%There is an undirected graph where the status of each vertex is either
%{\it active} or {\it inactive} at a time. An update involves switching the
%status of any vertex from active to inactive, or vice versa. The goal is to maintain a compact data structure that can efficiently answer connectivity query between any two vertices on the subgraph induced by the active vertices.
 
%Note that this is a weaker model as compared to fully dynamic connectivity under vertex updates.
%This is because the newly added vertices cannot be added with arbitrary edges. 
%Also any algorithm for fully dynamic connectivity under edge updates trivially solves dynamic subgraph connectivity
%at the expense of $O(n)$ factor in update time. This is because switching a vertex active or inactive is equivalent to $O(n)$ %edge updates. 


%There exists many efficient algorithms for the dynamic subgraph connectivity
%\cite{ChanPR08,Duan10,EppsteinGIN97,Frederickson85,HolmLT01,KapronKM13}. These algorithms offer different trade-offs between the update time and the query time, and differ on the types (amortized or worst case) of update time and
%the types (deterministic or randomized) of query time. 
%
%The best bound on the amrotized update time for the dynamic subgraph %connectivity is $min(O(m^{2/3}),\tilde{O}(n)))$ \cite{ChanPR08,HolmLT01}. %However, the best bound on the worst case update time for this problem is $min(O(m^{4/5}),O(n\sqrt{n}))$ \cite{Frederickson85,EppsteinGIN97,Duan10}. 
%It we can tolerate an error in query, there exists
%There exists 
%a worst case update time of $\tilde{O}(n)$ is also possible in the 
%randomized setting \cite{KapronKM13} at expense of error in output with a %probability which is inverse polynomial in terms of $n$. 
%Other relevant algorithms for subgraph connectivity are %\cite{Chan06,HenzingerK99}.
%
%The fastest update algorithm suitable for sparse graphs is by Chan, Patrascu, and Roditty \cite{ChanPR11} 
%taking $O(m^{2/3})$ amortized time per update and $O(m^{1/3})$ time per query. The fastest algorithm ensuring worst case
%guarantees is by Duan \cite{Duan10} taking $O(m^{4/5})$ time per update and $O(m^{1/5})$ time per query.
%For denser graphs fastest algorithms follows from solutions for dynamic connectivity for edge updates.
%The best algorithm is by Holm et al. \cite{HolmLT01} taking amortized $\tilde{O}(n)$ time per update.
%Fastest worst case update time algorithm was given by Frederickson \cite{Frederickson85} later improved by Eppstein et al. \cite{EppsteinGIN97} using sparsification technique taking $O(n\sqrt{n})$ time per update. 
%Better worst case update time is available in the randomized setting where Kapron et al. \cite{KapronKM13}
% achieves $\tilde{O}(n)$ update time at expense of error in output with a probability which is inverse polynomial in terms of $n$.
% 
%
%Chan, Patrascu, and Roditty \cite{ChanPR11} presented an algorithm for
%dynamic subgraph connectivity that achieves $\tilde{O}(m^{2/3})$ amortized update time and $\tilde{O}(m^{1/3})$ query time. 
%This result achieves the best amortized update time in terms of $m$ and is suitable for sparse graphs. 
%The fastest update time in terms of $n$ follows from solution of dynamic connectivity by Holm et al. \cite{HolmLT01} taking %amortized $\tilde{O}(n)$ time per update. The best worst case update time in terms of $m$ is achieved by Duan \cite{Duan10}
%taking $O(m^{4/5})$ time per update and $O(m^{1/5})$ time per query. In terms of $n$ the best worst case bound in deterministic
%setting is by Eppstein et al. \cite{EppsteinGIN97} which improves the algorithm by Frederickson \cite{Frederickson85} using sparsification technique. This algorithm takes $O(n\sqrt{n})$ time per update. If we allow the solution to err, the best update time in worst case is by Kapron, King, and Mountjoy \cite{KapronKM13} which achieves $\tilde{O}(n)$ update time at 
%the expense of error in output with a probablity which is inverse polynomial in terms of $n$.
%
%In the worst case scenario is due to a randomized algorithm by Kapron, King, and Mountjoy \cite{KapronKM13} for the fully dynamic connectivity problem.
%For dynamic subgraph connectivity problem, their algorithm implies 
%$\tilde{O}(n)$ worst case update time and $O(1)$ worst case query time. 
%However, the query alorithm may err with proability which is inverse polynomial in terms of $n$.
%
%The previous deterministic results for this problem that achieve $o(m)$ worst case update time are as follows. Duan \cite{Duan10} achieves $\tilde{O}(m^{4/5})$ update time and $O(m^{1/5})$ query time, and Eppstein et al. \cite{EppsteinGIN97} achieve $O(n\sqrt{n})$ update time and $O(1)$ query time. 
%We, as a direct application of our fully dynamic DFS tree algorithm, can achieve $\tilde{O}(\sqrt{mn})$ worst case update time and $O(1)$ query time 
%for the dynamic subgraph connectivity. 
%%However,
%%the best Our result also answers two open questions asked by Chan et al. \cite{ChanPR08}.
%%Our result is incomparable with the previously existing results stated above. 
%Moreover, our algorithm extends to dynamic subgraph bi-connectivity and dynamic subgraph 2-edge connectivity in a straightforward manner.
%, for which fully dynamic algorithms exist handling edge updates \cite{HolmLT01,EppsteinGIN97,Henzinger00}. Our results establish that it is indeed possible to achieve non-trivial bounds for the dynamic version of these fundamental problems using DFS tree approach. 
%Moreover our algorithm is far simpler as compared to previous results, making it an ideal candidate for practical 
%applications. 
%It will be interesting to see whether our algorithm can be suitably combined %with the previous algorithms to achieve alternate trade-offs between update %time and query time for these fundamental dynamic graph problems.


%We present an algorithm for the dynamic subgraph connectivity problem that takes $\tilde{O}(\sqrt{mn})$ worst case update time and $O(1)$
%deterministic query time. %Our result is incomparable with the previously existing results stated above. 
%Moreover, our algorithm extends to dynamic subgraph bi-connectivity and dynamic subgraph 2-edge connectivity in a straightforward manner. Our results establish that it is indeed possible to achieve non-trivial bounds for the dynamic version of these fundamental problems using DFS tree approach only. It will be interesing to
%see whether our algorithm may be suitably combined with the previous algorithms to achieve alternate trade-offs between update time and query time for the dynamic subgraph connectivity problem.

% 
%Our fully dynamic DFS tree directly provide extremely simple and
%efficient solution for dynamic sibgraph connectivity, connectivity, and 2-edge connectivity. 
%
%
%now present the applications of our fully dynamic DFS tree algorithm
%
%
%Dynamic Subgraph model is described as follows. 
%Given an undirected graph, the status of any vertex can be switched between  
%{\it active} and {\it inactive} in an update. The goal is to efficiently 
%answer the relevant query on the subgraph induced by the active vertices.
%Note that this is a weaker model as compared to fully dynamic vertex updates as the edges
%to the newly added vertices cannot be arbitrary. Also known algorithms for dynamic problems
%for edge updates can be used for these where one vertex update is performed by $O(n)$ edge updates.
%
%Dynamic subgraph connectivity is a well studied problem \cite{Chan06,ChanPR08,Duan10} with best 
%worst case update times $O(min(n\sqrt{n}$ \cite{Frederickson85,EppsteinGIN97}$,m^{4/5}$\cite{Duan10}$)$ 
%and best amortized bounds $O(n\log^2 n$ \cite{HolmLT01}$, m^{2/3}$ \cite{ChanPR08,Duan10}$)$. 
%
%There also exist a randomized algorithm with expected worst case update time of $O(n\log^5 n)$ \cite{KapronKM13}.
%Our dynamic DFS algorithm can seamlessly solve fully dynamic connectivity under vertex updates in
%deterministic worst case $O(\sqrt{mn}\log^{2.5} n)$ time per update with constant query time.
%
%
%\subsection*{Dynamic subgraph connectivity, bi-connectivity, and 2 edge-connectivity}
%The dynamic subgraph connectivity problem is defined as follows. Given
%an undirected graph, the status of any vertex can be switched between  
%{\it active} and {\it inactive} in an update. The goal is to efficiently 
%answer any on online connectivity query on the subgraph induced by the 
%active vertices. This problem can be solved using dynamic connectivity
%data structures \cite{EppsteinGIN97,Frederickson85,HolmLT01} that answers 
%connectivity queries under an online sequence of edge updates. This is 
%because switching the state of a vertex is equivalent to $O(n)$ edge 
%updates. Chan \cite{Chan06} introduced this problem and showed that it 
%can be solved more efficiently. He gave an algorithm using FMM (fast 
%matrix multiplication) that achieves $O(m^{0.94})$ amortized update time 
%and $\tilde{O}(m^{1/3})$ query time. Later Chan et al. \cite{ChanPR08} 
%presented a new algorithm that improves the amortized update time to 
%$\tilde{O}(m^{2/3})$. Further they established a lower bound of 
%$\Omega(\sqrt{m})$ time per update. They also mentioned the following 
%among the open problems.
%
%\begin{enumerate}
%\item
%Is it possible to achieve constant query time with worst case sublinear
%update time ?
%\item
%Can non trivial updates be obtained for richer queries such as counting
%the number of connected components ?
%\end{enumerate}
%
%Duan \cite{Duan10} answered the first question in affirmative but at the
%expense of much higher update time. We answer both these questions 
%affirmatively. Our fully dynamic algorithm directly provides an 
%$\tilde{O}(\sqrt{mn})$ update time and $O(1)$ query time algorithm for 
%the dynamic subgraph connectivity problem. Our algorithm maintains the
%number of connected components simply as a biproduct. In fact, our fully dynamic
%algorithm for DFS tree solves a generalization of dynamic subgraph connectivity 
%- in addition to just switching the status of vertices, it allows insertion of 
%new vertices as well.
%
%Exploiting the rich structure of DFS tree, we also obtain 
%$\tilde{O}(\sqrt{mn})$ update time algorithms for dynamic subgraph 
%bi-connectivity and dynamic subgraph 2 edge-connectivity in a seamless 
%manner. Figure \ref{figure:subGraph} illustrates our results and the 
%existing results in the right perspective. A variant of dynamic 
%subgraph connectivity problem has been studied by 
%Patrascu and Thorup \cite{PatrascuT07}. For any $k$ edge failures,
%their data structure takes $\tilde{O}(k)$ update time such that
%any subsequent connectivity query can be answered in $O(\log\log n)$ time.
%Later Duan and Pettie \cite{DuanP10} presented a data structure for vertex
%failures. For any $k$ vertex failures, their data structure takes 
%$\tilde{O}(k^6)$ update time and answers any subsequent 
%connectivity query in $O(k)$ time.
%
%%The connectivity problem 
%%have also been studied in the fault tolerant model by Patrascu and Thorup
%%\cite{PatrascuT07} for edge failures and by Duan and Pettie \cite{DuanP10} 
%%for vertex failures. The subgraph connectivity problem have also been studied
%%in the fault tolerant model. Patrascu and Thorup \cite{PatrascuT07} showed 
%%that one can answer connectivity queries after $d$ edge failures using 
%%$\tilde{O}(d)$ update time. Later Duan and Pettie \cite{DuanP10} improved 
%%this update time for $d$ vertex failures to $\tilde{O}(d^6)$. 
%Unlike all the previous algorithms for dynamic subgraph connectivity, which use heavy 
%machinery of existing dynamic algorithms, our algorithms are arguably much 
%simpler and self contained. 
%
%\begin{figure}[h!]
%\centering
%\def\arraystretch{0.6}
%\begin{tabular}{| m{4.5cm} | m{3.5cm} | m{2cm} | m{1.5cm} |}
%\hline
% {\bf References }							& {\bf Update Time} 					& {\bf Query Time} 		& {\bf Space} 			\\ \hline
%Frederickson \cite{Frederickson85} (1985), 
%Eppstein et. al \cite{EppsteinGIN97} (1997)\hfill$\dagger$& $O(n\sqrt{n})$  					& $O(1)$ 				& $O(m)$  				\\ \hline
%Holm et al. \cite{HolmLT01} (2001)\hfill$*\dagger$  		& $\tilde{O}(n)$ amortized  			& $\tilde{O}(1)$ 		& $O(m)$  				\\ \hline
%Chan  \cite{Chan06} (2006) 					& $\tilde{O}(m^{0.94})$ amortized	& $\tilde{O}(m^{1/3})$ 	& $\tilde{O}(m)$  		\\ \hline
%Chan et al. \cite{ChanPR08} (2008) 			& $\tilde{O}(m^{2/3})$ amortized		& $\tilde{O}(m^{1/3})$ 	& $\tilde{O}(m^{4/3})$ 	\\ \hline
%Duan \cite{Duan10} (2010) 					& $\tilde{O}(m^{2/3})$ amortized		& $\tilde{O}(m^{1/3})$ 	& $\tilde{O}(m)$  		\\ \hline
%Duan \cite{Duan10} (2010) 					& $\tilde{O}(m^{4/5})$ 				& $\tilde{O}(m^{1/5})$ 	& $\tilde{O}(m)$  		\\ \hline
%{\bf New\hfill $*\dagger$} 								& $\tilde{O}(\sqrt{mn})$ 			& $O(1)$ 				& $\tilde{O}(m)$  		\\ \hline
%\end{tabular}
%\caption{Current-state-of-the-art of the algorithms for the dynamic subgraph 
%connectivity. $(*)$ and $(\dagger)$ indicates that the result also solves subgraph bi-connectivity and 2-edge connectivity respectively.}
%\label{figure:subGraph}
%\end{figure}

% \subsection{Main Idea}
% % --Saying that we first consider the problem of k-updates?
% 
% The main idea behind breaking the $O(m)$ barrier is to avoid processing all the edges of the graph after a set of updates. This is possible by using a property of DFS traversal that we refer as the {\em components property}.
% To exploit this property we preprocess the DFS tree of the existing graph to form a data structure $\DD$.
% %It allows us to create a {\em reduced adjacency list} which is used by our algorithm.
% % It allows us to create a {\em reduced adjacency list} which on being used instead of the adjacency list
% % gives the same DFS tree.
% It allows us to create {\em reduced adjacency lists} which are sufficient to be scanned in 
% order to obtain a DFS tree of the updated graph.
% % In fact our algorithm resembles a lot with the static DFS algorithm, except that 
% % it uses and updates this reduced adjacency list as the graph is traversed. 
% These reduced adjacency lists are updated as the graph is traversed. 
% % However maintaining the data structure $\DD$ after every update is 
% % an expensive task, so we use a novel partitioning scheme to handle multiple failures (edges and vertices) 
% % using the original data structure.
% First we consider the case where the updates are only edge and vertex deletions.
% As a result we get a fault tolerant algorithm that can report the DFS tree
% efficiently after a batch of any $k$ failures.
% Later we show that this can be easily extended to handle insertions as well.
% Finally we convert this algorithm to a fully dynamic algorithm with worst case bounds using the
% standard overlapped rebuilding technique (also used by Thorup \cite{Thorup05} for maintaining fully 
% dynamic all pairs shortest paths). 
% % Reduced Adjacency list
% % Components property
% % Data structure
% % Fault tolerant Algorithm
% % Convert to fully dynamic and worst case
% 
% 
% \subsection{Organization of the paper}
% Remainder of the paper is divided into $7$ sections. Section \ref{sec:prelim} describes the various notations used throughout the paper. In Section \ref{sec:Overview}, we give an overview of our algorithm highlighting the main intuition behind our approach.
% Section \ref{sec:partition} describes a novel partitioning scheme used by our algorithm that is used to handle multiple updates at a time. Then in Section \ref{sec:algo} we present our algorithm that reports DFS tree efficiently after a batch of updates. 
% In Section \ref{sec:fullyDyn} we convert this algorithm to fully dynamic DFS and incremental DFS algorithms.
% In Section \ref{sec:apnIntro} and Section \ref{sec:Conclusion} we give a few applications and conclusion for our result.

\subsection{Main Idea}
Let $T$ be a DFS tree of $G$. To compute a DFS tree of $G+U$ for a given set
$U$ of updates, the main idea is to make use of the original tree $T$ itself. We preprocess the
graph $G$ using tree $T$ to build a data structure ${\cal D}$. In order
to achieve $o(m)$ update time, our algorithm makes use of ${\cal D}$ to create a {\it reduced} adjacency list
for each vertex such that performing DFS traversal using these lists gives a DFS tree for  $G+U$. 
%The algorithm essentially preforms a DFS traversal on $G+U$ cleverly using these {\it reduced} adjacency lists.
In fact, these reduced adjacency lists are generated on the fly and are guaranteed to have only $\tilde{O}(n|U|)$ edges. 

%\subsection{Outline of the paper}
We now give an outline of the paper.
In section \ref{sec:prelim}, we describe various notations used throughout the paper.
Section \ref{sec:Overview1} describes an algorithm to report the DFS tree after a single update in the graph.
The details of the required data structure $\DD$ are described in Section \ref{sec:data-structure}.
%provides an overview of our algorithm highlighting the main intuition behind our approach.
Then in Section \ref{sec:Overview2}, we provide an overview of our algorithm for handling 
multiple updates, highlighting the main intuition behind our approach.
%Section \ref{sec:Overview} provides an overview of our algorithm highlighting the main intuition behind our approach.
%In Section \ref{sec:partition} we describe a novel partitioning scheme used by our algorithm that is
%used to handle multiple updates at a time. 
Our main algorithm (Theorem \ref{main-result}) that reports a DFS tree after 
any set of updates in the graph is described in Section \ref{sec:algo}.
In Section \ref{sec:fullyDyn} we convert this algorithm to fully dynamic and incremental algorithms 
for maintaining a DFS tree using the \textit{overlapped periodic rebuilding} technique. 
%The details of the data structure $\DD$ are described in Section \ref{sec:data-structure}.
Finally, in Section \ref{sec:appn} and Section \ref{sec:LowerBounds} we describe the applications and 
lower bounds of dynamic DFS trees. 
% In Section \ref{sec:fullyDyn} we convert this algorithm to fully dynamic DFS and incremental DFS 
% algorithms. 
%In Section \ref{sec:Conclusion} we give conclusion for our result.


==> New folder/lowerBounds.tex <==
\section{Lower Bounds}
\label{sec:LowerBounds}
We now prove two conditional lower bounds for maintaining a DFS tree under vertex or edge updates.

\subsection{Vertex Updates}
The lower bound for maintaining a DFS tree under vertex updates is based on Strong Exponential Time Hypothesis (SETH) as defined below:
\begin{definition}[SETH]
For every $\epsilon>0$, there exists a positive integer $k$, such that SAT on $k-$CNF formulas on $n$ variables cannot be solved in $\tilde{O}(2^{(1-\epsilon)n})$ time.
\end{definition}

Given an undirected graph $G$ on $n$ vertices and $m$ edges in a dynamic environment (incremental / decremental or fully dynamic) under vertex updates.
The status of any vertex can be switched between  {\it active} and {\it inactive} in an update. 
The goal of subgraph connectedness is to efficiently answer whether the subgraph induced by active vertices is connected.
Abboud and Williams\cite{AbboudW14} proved a conditional lower bound of $\Omega(n)$ per update based on SETH for answering dynamic subgraph connectedness queries. 
They proved that any algorithm for answering dynamic subgraph connectedness queries using arbitrary polynomial preprocessing time and $O(n^{1-\epsilon})$ amortized update time would essentially refute the SETH conjecture. They also proved that any algorithm for maintaining partially dynamic (incremental/decremental) subgraph connectedness using arbitrary polynomial preprocessing time and  $O(n^{1-\epsilon})$ worst case update time would essentially refute the SETH conjecture.

We present a reduction from subgraph connectedness to maintaining DFS tree under vertex updates requiring the 
algorithm to report whether the number of children of the root in any DFS tree of the subgraph is greater than 1. 
Thus, we establish the following:

\begin{theorem}
Given an undirected graph $G$ with $n$ vertices and $m$ edges undergoing vertex updates, an algorithm for maintaining DFS tree that can report the 
number of children of the root in the DFS tree with preprocessing time $p(m,n)$, update time $u(m,n)$ and query time $q(m,n)$ would imply an algorithm 
for subgraph connectedness with preprocessing time $p(m+n,n)$, update time $u(m+n,n)$ and query time $q(m+n,n)$.
\end{theorem}

\begin{proof}
Given the graph $G$ for which we need to query for subgraph connectedness, we make a graph $G'$ as follows.
We add all vertices and edges of $G$ to $G'$. Further, add another vertex $r$ called as \emph{pseudo root} and connect it to all other vertices of $G'$.
Thus, $G'$ has $n+1$ vertices and $m+n$ edges.
Now, in any DFS tree $T$ of $G'$ rooted at $r$,  the number of children of $r$ will be equal to the number of components in $G$.
Here subtrees rooted on each child of $s$ represents a component of $G$.
Any change on $G$ can be performed on $G'$ and query for subgraph connectedness in $G$ is equivalent to querying if $r$ has more than 1 child in $T$.
\end{proof}

Thus, any algorithm for maintaining fully dynamic DFS under vertex updates with arbitrary preprocessing time and $O(n^{1-\epsilon})$ amortized update time would refute SETH. Also, any algorithm for maintaining partially dynamic DFS under vertex updates with arbitrary preprocessing time and $O(n^{1-\epsilon})$ worst case update time would refute SETH. 

\subsection{Edge Updates}
We now present a lower bound for maintaining a DFS tree under edge updates that holds for any algorithm which maintains tree edges of the DFS tree explicitly.
In the following example we prove that there exists a graph $G$ and a sequence of edge updates $U$, such that any DFS tree of the graph would 
require a conversion of $\Omega(n)$ edges from tree edges to back edges and vice-versa after every pair of updates in $U$. 

\begin{figure}[ht]
	\hspace{1cm}\includegraphics[width=.8\linewidth]{Figures/worstCase2.pdf}
	\caption{Worst Case Example for lower bound on maintaining DFS tree under fully dynamic edge updates.}

	\label{fig:worstCase}
\end{figure}



Consider the following graph for which a DFS tree rooted at $r$ is to be maintained under fully dynamic edge updates. 
There are $n/2$ vertices $u_1$,...,$u_l$ that have edges to vertices $x$ and $y$.
The remaining $n/2-3$ vertices $v_1$,..., $v_k$ are connected in form of a line as shown in Figure \ref{fig:worstCase}.
At any point of time one of $v_1,...,v_k$ (say $v_1$) is connected to either $x$ or $y$. %Let $v_1$ be the vertex connected to $y$.
The DFS tree for the graph is shown in Figure \ref{fig:worstCase} (i). Now, upon insertion of edge $(v_i,x)$ (say $i=2$) and deletion of edge $(v_1,y)$
the DFS tree will transform to either Figure \ref{fig:worstCase} (ii) or Figure \ref{fig:worstCase} (iii). Clearly $\Omega(n)$ edges are converted from tree edges to back edges and vice-versa. 
This can be repeated alternating between $x$ and $y$ ensuring that the new DFS tree 
requires $\Omega(n)$ after every two edge updates. 
Further, we repeat this for different $v_i$'s ensuring that the new DFS tree is not exactly 
the same as some previous DFS tree (thus memorization of the complete tree will not help).
Note that the same procedure can be applied to both the possible trees shown in Figure~\ref{fig:worstCase}(ii) and Figure~\ref{fig:worstCase}(iii).
%This can be repeated for any $v_i$ alternating between $x$ and $y$ ensuring that the new DFS tree is not exactly the same as some
%previous DFS tree (thus memorization of the complete tree will not help). 
Hence any algorithm maintaining tree edges explicitly takes $\Omega(n)$ time to handle such a pair of edge updates. 

==> New folder/overview.tex <==
\subsection{Properties of a DFS tree}
%\section{Handling a single update}
%\label{sec:Overview1}
DFS traversal has the following flexibility : when the traversal reaches  a vertex, say $v$, the next vertex 
to be traversed can be {\em any} unvisited neighbor of $v$. 
%Exploiting this flexibility, we can rebuild the DFS tree efficiently after an update using the following property
%of DFS traversal.
In order to compute a DFS tree for $G+U$ efficiently, our algorithm exploits this flexibility,
the original DFS tree $T$, and the following property of DFS traversal. 

\begin{figure}[!hb]
\centering
\includegraphics[width=0.35\linewidth]{Figures/components2.pdf}
\caption{Edges $e_1'$ as well as $e_2'$ can be ignored during the DFS traversal.}
\label{fig:component-property}
\end{figure}

\begin{lemma}[Components Property]
\label{lemma:L()}
%Let $v$ be a vertex that any DFS traversal is visiting currently and $T^*$ be the partially grown DFS tree. 
Let $T^*$ be the partially grown DFS tree and $v$ be the vertex currently being visited. 
Let $C$ be any connected component in the subgraph induced by the unvisited vertices.  Suppose two edges $e$ and $e'$ from $C$
are incident respectively on $v$ and some ancestor (not necessarily proper) $w$ of $v$ in $T^*$. Then it is sufficient to 
consider only $e$ during the rest of the DFS traversal, i.e., the edge $e'$ need not  be scanned. (Refer to Figure \ref{fig:component-property}).
\end{lemma}


Skipping $e'$ during the DFS traversal, as stated in the components property, is justified because $e'$ will appear
as a back edge in the resulting DFS tree. A similar property describing the \textit{inessential} edges of a DFS trees 
was used by Smith~\cite{Smith86} for computing a DFS tree of a planar graph in the parallel setting.
In order to highlight the importance of the components property, and to motivate the requirement of data structure $\cal D$,
we first consider a simpler case which deals with reporting a DFS tree after a single update in the graph.

\section{Handling a single update}
\label{sec:Overview1}


Consider the failure of a single edge $(b,f)$ (refer to Figure \ref{figure:overview-failure-eg} (i)).
Exploiting the flexibility of DFS traversal, we can assume a stage in the DFS traversal of $G\backslash \{(b,f)\}$ where
the partial DFS tree $T^*$ is $T\backslash T(f)$ and  vertex $b$ is currently being visited. 
Thus, the unvisited graph is a single connected component containing the vertices of $T(f)$. 
Now, according to the components property we need to process only the lowest edge from $T(f)$ to $path(b,r)$ 
($(k,b)$ in Figure \ref{figure:overview-failure-eg} (ii)). 
Hence, the DFS traversal enters this component using the edge $(k,b)$ and performs a traversal of the subgraph induced by the vertices of $T(f)$.
The resulting DFS tree of this subgraph would now be rooted at $k$. 
Rebuilding the DFS tree after the failure of edge $(b,f)$ thus reduces to 
finding the lowest edge from $T(f)$ to $path(e,r)$, 
and then rerooting a subtree $T(f)$ of $T$ at the new root $k$. 
We now describe how this rerooting can be performed in $\tilde{O}(n)$ time
in the following section.


\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/overview_failure_eg3.pdf}
\caption{ (i) Failure of edge $(b,f)$. 
(ii) Partial DFS tree $T^*$ with unvisited graph $T(f)$, component property allows us to neglect $(a,l)$.
(iii) Augmented $path(k,f)$ to $T^*$, the components property allows us to neglect $(l,k)$.
(iv) Final DFS tree of $G\backslash \{(b,f)\}$.
}
\label{figure:overview-failure-eg}
\end{figure}

\subsection{Rerooting a DFS tree}
Given a DFS tree $T$ originally rooted at $r_0$ and a vertex $r'$, 
the aim is to compute a DFS tree of the graph that is rooted at $r'$. 
Note that any subtree $T(x)$ of the DFS tree $T$ is also a DFS tree of the subgraph
induced by the vertices of $T(x)$. Hence, the same procedure can be 
applied to reroot a subtree $T(x)$ of the DFS tree $T$. 
%Thus in general we aim at rerooting $T(r_0)$ to a new root $r'\in T(r_0)$ 
Thus, in general our aim is to reroot $T(r_0)$ at a new root $r'\in T(r_0)$ 
(see Figure \ref{figure:overview-failure-eg} (ii), where the subtree 
$T(f)$ would be rerooted at its new root $k$).

\begin{figure*}[!ht]
%\begingroup
\centering
\begin{procedure}[H]
\BlankLine
\ForEach(\tcc*[f]{$a=par(b)$ in original tree $T(r_0)$.}){$(a,b)$ on $path(r_0,r')$}
	{
	$par(a)\leftarrow b$\;
	\ForEach{child $c$ of $b$ not on $path(r_0,r')$}
		{
		$(u,v)\leftarrow Query(T(c),r_0,b)$
		\tcc*{where $u\in path(r_0,r')$ and $v\in T(c)$.} 
		\If{$(u,v)$ is non-null}
			{
%			Delete $(b,c)$ from $T$\;
%			Add $(u',v')$ to $T$\;
			$Reroot(T(c),v)$\;
			$par(v)\leftarrow u$\;
			}
		}	
}
\caption{Reroot(\text{$T(r_0),r'$}): Reroots the subtree $T(r_0)$ of $T$ to be rooted at the vertex $r'\in T(r_0)$.}
%\caption{Reroot($T(r_0),r'$): Reroots the subtree $T(r_0)$ of $T$ to be rooted at the vertex $r'$.}
\label{alg:re-root}
\end{procedure}
\caption{The recursive algorithm to reroot a DFS tree $T(r_0)$ at the new root $r'$.}
\end{figure*}


Our algorithm (refer to Procedure \ref{alg:re-root}) essentially performs %guides 
the DFS traversal (exploiting the flexibility of DFS) %such
in such a way
that components of the unvisited graph can be easily identified.
The components property can then be applied to each such component, processing only $O(n)$ edges 
to compute the rerooted DFS tree.
The DFS traversal first visits the path from $r'$ to the root of tree $T(r_0)$. 
This reverses $path(r_0,r')$ in the new DFS tree $T^*$ as now $r'$ would be an ancestor of $r_0$ (see Figure \ref{figure:overview-failure-eg} (iii)).
Now, each subtree hanging from $path(r',r_0)$ in $T$ forms a component of the unvisited graph. 
This is because the presence of any edge between these subtrees would imply a cross edge in the original DFS tree. 
Using the components property we know that for each of these subtrees, say $T_i$,  
we only need to process the lowest edge from $T_i$ on the new path from $r'$ to $r_0$ in $T^*$.
Since $path(r',r_0)$ is reversed in $T^*$, it is equivalent to processing the highest edge 
$e_i$ from $T_i$ to the $path(r_0,r')$ in $T$. Recall that this query can be answered by our data structure $\cal D$
in $O(\log^3 n)$ time (refer to Section \ref{sec:prelim}). Now, let $v_i$ be the end vertex of $e_i$ in $T_i$.
The DFS traversal will thus visit the component induced by the vertices of $T_i$ through $e_i$,
and produces its DFS tree that is rooted at $v_i$. This rerooting can be performed by invoking the rerooting procedure
recursively on the subtree $T_i$ with the new root $v_i$.


%Given a DFS tree (or its subtree $T(f)$) originally rooted at $r_0$ (here $f$), the aim is to rebuild this DFS tree which is now rooted at 
%some vertex $r'$ (here $k$). The traversal first enters the component using $r'$ and traverses the path to the root of this DFS tree $r_0$.
%Now, the subtrees hanging from $path(r',r_0)$ forms the components of the unvisited graph ($T(h)$ and $T(l)$ in Figure \ref{figure:overview-failure-eg} (iii)). 
%This is because presence of any edge between these subtrees would imply a cross edge in the original DFS tree. 
%Using the components property we know that for each of these subtrees (say $T_i$) we find the lowest edge from $T_i$ to $path(r',r_0)$.
%Note that since $path(r',r_0)$ is reversed in $T^*$ as compared to $path(r_0,r')$ in $T$, 
%it is equivalent to find the highest edge $e_i$ from $T_i$ on $path(r_0,r')$ in $T$.
%Now, each $T_i$ would be rerooted independent of each other on the new root (end point of $e_i$ in $T_i$) when the DFS traversal enters 
%$T_i$ using the edge $e_i$. This process continues using recursively rerooting subtrees of $T$ until every vertex is visited. 



We now analyze the total time required by Procedure \ref{alg:re-root} to reroot a subtree $T'$ of the DFS tree $T$. 
The total time taken by our algorithm is proportional to the number of edges processed by the algorithm.
These edges include the {\em tree edges} that were a part of the original tree $T'$ and 
the {\em added edges} that are returned by the data structure $\cal D$.
Clearly, the number of tree edges in $T'$ are $O(|T'|)$. Also, since the added edges eventually become 
a part of the new DFS tree $T^*$, they too are bounded by the size of the tree $T'$. 
Further, the data structure $\cal D$ takes $O(\log^3 n)$ time to report each added edge. 
Hence the total time taken by our algorithm to rebuild $T'$ is $O(|T'|\log^3 n)$ time. 
Since $\cal D$ can be built in $O(m\log n)$ time (refer to Theorem \ref{thm:DS} in the Section \ref{sec:data-structure}),
we have the following theorem.  

% 
%The total time required to reroot a DFS tree is thus dependent on how efficiently we can find the lowest/highest edge from a subtree of $T$
%to some path in $T$. In section \ref{sec:data-structure} we describe a data structure $\cal D$ that preprocesses the graph $G$ and the DFS tree $T$
%in $O(m\log n)$ time to allow us to find such an edge in $O(\log ^3 n)$ time.
%The total edges processed by our algorithm are limited to the ones returned by our data structure, which eventually becomes a part of the new DFS tree $T^*$.
%These edges are limited to size of $T'$, hence the total time taken by our algorithm to rebuild $T'$ is $O(|T'|\log^3 n)$ time. Thus we have the following lemma.  

\begin{theorem}
An undirected graph can be preprocessed to build a data structure in $O(m \log n)$ time, such that 
any subtree $T'$ of the DFS tree can be rerooted at any vertex in $T'$, in $O(|T'| \log^3 n)$ time.
\label{thm:reroot}
\end{theorem}

%Thus the DFS tree can be rebuilt after an edge deletion in $\tilde{O}(n)$ time.
We now formally describe how rebuilding a DFS tree after an update can be reduced 
to this simple rerooting procedure (see Figure \ref{figure:overview-updates}). 
\begin{enumerate}
\item \textbf{Deletion of an edge $(u,v)$:}\\
In case $(u,v)$ is a back edge in $T$, simply delete it from the graph.
Otherwise, let $u = par(v)$ in $T$. 
The algorithm finds the lowest edge $(u',v')$ on the $path(u,r)$ from $T(v)$, where $v'\in T(v)$. 
The subtree $T(v)$ is then rerooted at its new root $v'$ and hanged from $u'$ using $(u',v')$ in the final tree $T^*$.
\item \textbf{Insertion of an edge $(u,v)$:}\\
In case $(u,v)$ is a back edge, simply insert it in the graph.
Otherwise, let $w$ be the LCA of $u$ and $v$ in $T$ and $v'$ be the child of $w$ such that $v\in T(v')$.
The subtree $T(v')$ is then rerooted at its new root $v$ and hanged from $u$ using $(u,v)$ in the final tree $T^*$.
\item \textbf{Deletion of a vertex $u$:}\\
Let $v_1,...,v_c$ be the children of $u$ in $T$. 
For each subtree $T(v_i)$, the algorithm finds the lowest edge $(u'_i,v'_i)$ on the $path(par(u),r)$ from $T(v_i)$, where $v'_i\in T(v_i)$. 
Each subtree $T(v_i)$ is then rerooted at its new root $v'_i$ and hanged from $u'_i$ using $(u'_i,v'_i)$ in the final tree $T^*$.
\item \textbf{Insertion of a vertex $u$:}\\
Let $v_1,...,v_c$ be the neighbors of $u$ in the graph. 
Make $u$ a child of some $v_j$ in $T^*$.
%Arbitrarily choose a neighbor $v_j$ and make $u$ the child of $v_j$ in $T^*$. 
For each $v_i$, such that $v_i\notin path(v_j,r)$, let $T(v'_i)$ be the subtree hanging from $path(v_j,r)$
such that $v_i\in T(v'_i)$. %In case $v'_{i_1} = v'_{i_2}$, ignore any one of the corresponding $v_{i_1}$ or $v_{i_2}$.
Each subtree $T(v'_i)$ is then rerooted at its new root $v_i$ and 
hanged from $u$ using $(u,v_i)$ in the final tree $T^*$.
\end{enumerate}

%Further the reader may note that several other kinds of updates in the graph as insertion of an edge, insertion/deletion of a vertex etc.
%can also be reduced to this simple rerooting procedure.

\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/overview_reroot2.pdf}
\caption{Updating the DFS tree after a single update: (i) deletion of an edge, (ii) insertion of an edge, 
(iii) deletion of a vertex, and (iv) insertion of a vertex. 
The reduction algorithm reroots the marked subtrees (shown in violet) and hangs it from the 
inserted edge (in case of insertion) or the lowest edge (in case of deletion) on the marked path 
(shown in blue) from the marked subtree.
%The algorithm reroots the marked subtrees (marked in violet) and hangs it from the inserted edge (in case of insertion)
%or the lowest edge (in case of deletion) on the marked path (marked in blue) from the marked subtree.
%In case of insertion the rerooted subtree is hanged from the inserted edge.
%or the lowest edge (in (i) and (iii)) from the marked subtree to the marked path (marked in blue). 
}
\label{figure:overview-updates}
\end{figure}

In case of vertex updates, multiple subtrees may be rerooted by the algorithm. Let these subtrees be $T_1,...,T_c$.
Thus, the total time taken by our algorithm is equal to the time taken to reroot the subtrees $T_1,...,T_c$.  
Using Theorem \ref{thm:reroot}, we know that a subtree $T'$ can be rerooted in $\tilde{O}(|T'|)$ time.
Since these subtrees are disjoint, the total time taken by our algorithm to build the resulting DFS tree is 
$\tilde{O}(|T_1|+...+|T_c|) = \tilde{O}(n)$. 
Thus, we have the following theorem.

\begin{theorem}
An undirected graph can be preprocessed to build a data structure in $O(m \log n)$ time such that 
after a single update in the graph, the DFS tree can be reported in $O(n \log^3 n)$ time.
\label{thm:DFS_reroot}
\end{theorem}

%In the following section we describe how to build the data structure $\cal D$ used by our algorithm. 

%However, the time required to build the data structure $\cal D$ is $O(m\log n)$, hence it cannot be rebuild after every update in the DFS tree. 
%Thus, in order to handle a sequence of updates our aim is to handle multiple updates together without having to rebuild the data structure after every update.
%This gives a fault tolerant algorithm for the problem described as follows.

\begin{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 14Nov Version %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Overview}
\label{sec:Overview}
Static DFS traversal explores each edge in the graph and thus takes $\Theta(m+n)$ time. 
In order to compute the DFS tree for $G+U$ in $o(m)$ time, the aim is 
to explore only a {\em small} subset of neighbors $L(v)\subseteq N(v)$ of every vertex $v$. 
For this purpose, 
%DFS traversal has the following flexibility : when the traversal reaches  a vertex, say $v$, the next vertex 
%to be traversed can be {\em any} unvisited neighbor of $v$. 
%In order to compute a DFS tree for $G+U$ efficiently, our algorithm exploits this flexibility,
%the original DFS tree $T$, and the following property of DFS traversal.
we exploit the flexibility inherent in DFS traversal 
and an important property. The flexibility of DFS is that once traversal reached a 
vertex $v$, the next vertex to be traversed can be any one among its unvisited 
neighbors. We also exploit the following property of DFS traversal.
%Following We now state the important property of DFS traversal.


\begin{figure}[!hb]
\centering
\includegraphics[width=0.35\linewidth]{Figures/components2.pdf}
\caption{Edges $e_1'$ as well as $e_2'$ can be ignored during the DFS traversal.}
\label{fig:component-property}
\end{figure}

\begin{lemma}[Components Property]
\label{lemma:L()}
%Let $v$ be a vertex that any DFS traversal is visiting currently and $T^*$ be the partially grown DFS tree. 
Let $T^*$ be the partially grown DFS tree and $v$ be the vertex currently visited. 
Let $C$ be any connected component in the subgraph induced by the unvisited vertices.  Suppose two edges $e$ and $e'$ from $C$
are incident respectively on $v$ and some ancestor (not necessarily proper) $w$ of $v$ in $T^*$. Then it is sufficient to 
consider only $e$ during the rest of the DFS traversal, i.e., the edge $e'$ need not  be scanned. (Refer to Figure \ref{fig:component-property}).
\end{lemma}

Skipping $e'$ during the DFS traversal, as stated in the components property, is justified because $e'$ will appear
as a back edge in the resulting DFS tree. 
%Let us now understand how this property can be used to handle a single update in a graph. %, reporting the resulting DFS tree in $\tilde{O}(n)$ time.
In order to have a deeper insight of the components property let us consider a simpler update.
Consider the failure of a single edge $(b,f)$ (refer to Figure \ref{figure:overview-failure-eg} (i)).
Exploiting the flexibility of DFS traversal, we can assume a stage in the DFS traversal of $G\backslash \{(b,f)\}$ where
the partial DFS tree $T^*$ is $T\backslash T(f)$. Note that the unvisited graph is a single connected component
containing the vertices in $T(f)$. Now, using components property we find only the lowest edge from $T(f)$ on $path(e,r)$
($(k,b)$ in Figure \ref{figure:overview-failure-eg} (ii)). Hence entering the component represented by the vertices of $T(f)$,
the DFS traversal rebuilds the DFS tree of the subgraph induced by $T(f)$ which is now rooted at $k$. 
We now describe how this rerooting can be performed recursively to report the resulting DFS tree in $\tilde{O}(n)$ time.


\begin{figure}[!ht]
\centering
\includegraphics[width=.8\linewidth]{Figures/overview_failure_eg3.pdf}
\caption{ (i) Failure of edge $(b,f)$. 
(ii) Partial DFS tree $T^*$ with unvisited graph $T(f)$, component property allows us to neglect $(a,l)$.
(iii) Augmented $path(k,f)$ to $T^*$, components property allows us to neglect $(l,k)$.
(iv) Final DFS tree of $G\backslash \{(b,f)\}$.
}
\label{figure:overview-failure-eg}
\end{figure}

\subsection*{Rerooting a DFS tree}
Given a DFS tree (or its subtree $T(f)$) originally rooted at $r_0$ (here $f$), the aim is to rebuild this DFS tree which is now rooted at 
some vertex $r'$ (here $k$). The traversal first enters the component using $r'$ and traverses the path to the root of this DFS tree $r_0$.
Now, the subtrees hanging from $path(r',r_0)$ forms the components of the unvisited graph ($T(h)$ and $T(l)$ in Figure \ref{figure:overview-failure-eg} (iii)). 
This is because presence of any edge between these subtrees would imply a cross edge in the original DFS tree. 
Using the components property we know that for each of these subtrees (say $T_i$) we find the lowest edge from $T_i$ to $path(r',r_0)$.
Note that since $path(r',r_0)$ is reversed in $T^*$ as compared to $path(r_0,r')$ in $T$, 
it is equivalent to find the highest edge $e_i$ from $T_i$ on $path(r_0,r')$ in $T$.
Now, each $T_i$ would be rerooted independent of each other on the new root (end point of $e_i$ in $T_i$) when the DFS traversal enters 
$T_i$ using the edge $e_i$. This process continues using recursively rerooting subtrees of $T$ until every vertex is visited. 
 
The total time required to reroot a DFS tree is thus dependent on how efficiently we can find the lowest/highest edge from a subtree of $T$
to some path in $T$. In section \ref{sec:data-structure} we describe a data structure $\cal D$ that preprocesses the graph $G$ and the DFS tree $T$
in $O(m\log n)$ time to allow us to find such an edge in $O(\log ^3 n)$ time.
The total edges processed by our algorithm are limited to the ones returned by our data structure, which eventually becomes a part of the new DFS tree $T^*$.
These edges are limited to size of $T'$, hence the total time taken by our algorithm to rebuild $T'$ is $O(|T'|\log^3 n)$ time. Thus, we have the following lemma.  

\begin{lemma}
An undirected graph can be preprocessed to build a data structure in $O(m \log n)$ time such that 
any subtree $T'$ of the DFS tree can be rebuild to be rooted at some vertex in $T'$ in $O(|T'| \log^3 n)$ time.
\label{lemm:reroot}
\end{lemma}

Thus the DFS tree can be rebuilt after an edge deletion in $\tilde{O}(n)$ time.
Further the reader may note that several other kinds of updates in the graph as insertion of an edge, insertion/deletion of a vertex etc.
can also be reduced to this simple rerooting procedure.
However, the time required to build the data structure $\cal D$ is $O(m\log n)$, hence it cannot be rebuild after every update in the DFS tree. 
Thus in order to handle a sequence of updates our aim is to handle multiple updates together without having to rebuild the data structure after every update.
This gives a fault tolerant algorithm for the problem described as follows.

\subsection*{Fault tolerant DFS}
Instead of querying just the edges required to be added to $T^*$ we build a {\em reduced adjacency list} for the graph such that 
DFS traversal using these sparser lists gives the DFS tree of the updated graph.
%The components property is exploited to compute these reduced adjacency lists for building a DFS tree as follows.
Consider a set $U$ of updates, we compute a partitioning of $T$ into 
a disjoint collection of ancestor-descendant paths and subtrees
such that none of these subtrees and paths contain any failed edge or vertex. 
An important property of this partitioning is that there are no edges from $G$ lying between
any two subtrees in this partitioning. We refer to this partitioning as a {\em disjoint tree partitioning}.
In fact, this partitioning depends upon only the vertex and edge failures in the set $U$.

Recall that during the DFS traversal we need to find the lowest edge from each component $C$ of the unvisited graph.
It turns out that each component $C$ can be represented as a union of subtrees and ancestor-descendant paths of the original DFS tree $T$. 
%Furthermore, there exists a data structure $\DD$ that can efficiently report the lowest edge from the subtrees and the ancestor-descendant paths to $p_0$.
The components property can now be employed to compute the reduced adjacency lists of the graph as follows.
%Thus we employ the components property to 
We just find the lowest edge from each of the subtrees and the ancestor-descendant paths to $T^*$ by querying the data structure $\DD$.
Let this edge be $(x,y)$ where $x\in T^*$ and $y\in C$. We can just add $y$ to the reduced adjacency list $L(x)$ of $x$.
Since components property ensures the remaining edges to $T^*$ can be ignored, the DFS traversal would thus consider all possible 
candidates for the lowest edge from $C$ to $T^*$.
Let the initial disjoint tree partitioning consists of a set of ancestor-descendant paths ${\cal P}$ 
and a set of subtrees ${\cal T}$. The algorithm for computing a DFS tree of $G+U$ can be summarized as follows:

{\em Perform the static DFS traversal on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices.
%The algorithm for computing a DFS tree of $G+U$ is quite similar
%to the static DFS traversal executed on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices as follows.
%the wherein we grow $L(v)$ for each vertex $v$ lazily and cleverly as follows.
%Consider each element of ${\cal P}\cup{\cal T}$ as a {\em super} vertex.
Visiting a super vertex $v^*$ by the algorithm involves extracting an ancestor-descendant path $p_0$ 
%of $T$ is extracted 
from $v^*$ and attaching it to the partially grown DFS tree $T^*$. The remaining part of 
$v^*$ is added back to $\PP \cup \TT$ as {\em new} super vertices.
% maintaining the properties of disjoint tree partition. 
Thereafter, the reduced adjacency list of the vertices on path $p_0$ is computed using the data structure
$\DD$. The algorithm then continues to find the next super vertex using the reduced adjacency lists. }






\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBMITTED SODA VERSION %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Static DFS traversal has to explore each edge and thus needs $\Theta(m+n)$ 
%time. In order to compute the DFS tree for $G+U$ in $o(m)$ time, the aim is 
%to explore only a {\em small} subset of neighbors $L(v)\subseteq N(v)$ of every 
%vertex $v$. For this purpose, 
DFS traversal has the following flexibility : when the traversal reaches  a vertex, say $v$, the next vertex 
to be traversed can be {\em any} unvisited neighbor of $v$. 
In order to compute a DFS tree for $G+U$ efficiently, our algorithm exploits this flexibility,
the original DFS tree $T$, and the following property of DFS traversal.
%
%We exploit the flexibility inherent in DFS traversal 
%and an important property. The flexibility of DFS is that once traversal reached a 
%vertex $v$, the next vertex to be traversed can be any one among its unvisited 
%neighbors of $v$. We now state the important property of DFS traversal.
%


\begin{figure}[!hb]
\centering
\includegraphics[width=0.35\linewidth]{Figures/components2.pdf}
\caption{Edges $e_1'$ as well as $e_2'$ can be ignored during the DFS traversal.}
\label{fig:component-property}
\end{figure}

\begin{lemma}[Components Property]
\label{lemma:L()}
%Let $v$ be a vertex that any DFS traversal is visiting currently and $T^*$ be the partially grown DFS tree. 
Let $T^*$ be the partially grown DFS tree and $v$ be the vertex currently visited. 
Let $C$ be any connected component in the subgraph induced by the unvisited vertices.  Suppose two edges $e$ and $e'$ from $C$
are incident respectively on $v$ and some ancestor (not necessarily proper) $w$ of $v$ in $T^*$. Then it is sufficient to 
consider only $e$ during the rest of the DFS traversal, i.e., the edge $e'$ need not  be scanned. (Refer to Figure \ref{fig:component-property}).
\end{lemma}

Skipping $e'$ during the DFS traversal, as stated in the components property, is justified because $e'$ will appear
as a back edge in the resulting DFS tree.
%-------------------8July  begins-------
%To understand the main intuition behind the components property, consider the instance when 
%DFS traversal reaches a vertex $v$. Let $H$ be the unvisited graph at this instance, and 
%$(v,x)$ be the first edge scanned by $v$ that is incident to it from component $C$.
%As a result $x$ becomes a child of $v$. Now note that the DFS traversal on reaching $x$ is like 
%a fresh DFS from $x$ in the graph $H$. Thus, at the time when DFS traversal finishes for
%vertex $x$, all the vertices that were reachable from $x$ in $H$ (this is essentially 
%set $C$) lie in subtree under $x$.
%Let $e'=(w,x')$ where $w$ an ancestor of $v$ and $x' \in C$
%Since w is an ancestor of x, we have that e' is a back edge in the final DFS tree.
%-----------------8-July ends----------
%
%
% Hence, from each component we only need to find the lowest (??) edge (say $(u,v)$ where $u\in T^*$)
% incident on the partially build DFS tree and add $v$ to the reduced adjacency list $L(u)$ of $u$.
%
% Consider a path $p_0$ in the partially built DFS tree $T^*$ for whose vertices we need to 
% compute reduced adjacency list. By Lemma \ref{lemma:L()} from each component $C$ of the unvisited 
% graph we only need to find a lowest edge incident on $p_0$ (say $(u,v)$ where $u\in p_0$, and $v\in C$)
% and add $v$ to the reduced adjacency list $L(u)$ of $u$.
% 
The components property can be exploited to compute reduced adjacency lists of small size for building a DFS tree as follows.
Let $p_0$ be the path from the root to $v$ in the partially built DFS tree $T^*$.
%The components property implies the existence of reduced adjacency lists of small size as follows. Let $p_0$ be the path
%from the root to $v$ in the partially built DFS tree $T^*$.
% for whose vertices we need to 
%compute reduced adjacency list. By Lemma \ref{lemma:L()} 
From each component $C$ of the unvisited graph, we only need to find an edge incident to the lowest vertex on $p_0$.
Let this edge be $(x,y)$ where $x\in p_0$ and $y\in C$. We can just add $y$ to the reduced adjacency list $L(x)$ of $x$ and ignore
all other edges incident from $C$ to $p_0$.
%
% Consider a path $p_0$ in the partially built DFS tree $T^*$ for whose vertices we need to 
% compute reduced adjacency list. By Lemma \ref{lemma:L()} from each component $C$ of the unvisited 
% graph we only need to find a lowest vertex on $p_0$ adjacent to $C$, say $u$,
% and add a vertex from $N(u)\cap C$ to reduced adjacency list $L(u)$.
%
% In order to understand our algorithm we first consider the stack based standard DFS algorithm.
% In it whenever a vertex $u$ is visited for the first time by the traversal it is pushed 
% into stack $S$, and the whole adjacency list of $u$ is scanned before it is popped out. 
% In order to compute the DFS tree for a graph after a given set of updates we perform a
% modified DFS traversal of it as follows. Whenever a vertex $u$ is visited for the first 
% time, then instead of just attaching $u$ to the tree, we extract a path $p_0$ (starting 
% from $u$) from the unvisited graph an attach it to partially built DFS tree. 
% We exploit here the flexibility of DFS traversal that on reaching a vertex $u$ it can 
% follow any arbitrary path in the unvisited graph.
% We mark the vertices of $p_0$ as visited and also push them in the stack.
% Next we compute the reduced adjacency list of vertices belonging to path $p_0$.
% For each component $C$ in the unvisited graph we ensure that if $w$ is the 
% lowest vertex on path $p_0$ (i.e. vertex farthest from root) which is adjacent to $C$,
% then at least one vertex from $N(w)\cap C$ is added to set $L(w)$.
% It turns out that the reduced adjacency lists constructed in this fashion are sufficient
% to be scanned in order to obtain a valid DFS tree.
%
%
%The task of computing the reduced adjacency lists efficiently is accomplished
%using the original DFS tree $T$ as follows.
However, as the reader may also observe, maintaining the connected components 
of the unvisited graph and obtaining the lowest edge incident from each of them to $p_0$ is a non-trivial task. 
Nevertheless, we are able to accomplish this task by exploiting the original DFS tree $T$ of $G$ as follows. 

%----------commented on 13October
%We compute and maintain a partitioning of the unvisited graph into 
%a disjoint collection of ancestor-descendant paths and subtrees of $T$  
%such that none of these subtrees and paths contain any failing edge or vertex. 
%We refer to this partitioning as a {\em disjoint tree partitioning}.
%An important property of this partitioning is that there are no edges from $G+U$ lying between
%any two subtrees in ${\cal T}$. 
%It turns out that each component $C$ of the unvisited graph during a DFS traversal can be represented 
%as a union of  subtrees and ancestor-descendant paths of the original DFS tree $T$. 
%Furthermore, there exists a data structure $\DD$ that can efficiently report the lowest edge from the subtrees and the ancestor-descendant paths to $p_0$.
%The lowest edges from the subtrees and the ancestor-descendant paths is then obtained by querying the %data structure $\DD$.

For a given set $U$ of updates, we compute a partitioning of $T$ into 
a disjoint collection of ancestor-descendant paths and subtrees
such that none of these subtrees and paths contain any failed edge or vertex. 
An important property of this partitioning is that there are no edges from $G$ lying between
any two subtrees in ${\cal T}$. We refer to this partitioning as a {\em disjoint tree partitioning}.
Note that this partitioning depends upon only the vertex and edge failures in the set $U$.
It turns out that each component $C$ of the unvisited graph during a DFS traversal can be represented 
as a union of subtrees and ancestor-descendant paths of the original DFS tree $T$. 
%Furthermore, there exists a data structure $\DD$ that can efficiently report the lowest edge from the subtrees and the ancestor-descendant paths to $p_0$.
The lowest edges from the subtrees and the ancestor-descendant paths can be obtained by querying the data structure $\DD$.

%With insights from the disjoint tree partitioning and the component property at its core, 
%our algorithm now exploits the flexibility of the DFS traversal to compute the DFS tree of $G+U$ as %follows.
Let the initial disjoint tree partitioning consists of a set of ancestor-descendant paths ${\cal P}$ 
and a set of subtrees ${\cal T}$. The algorithm for computing a DFS tree of $G+U$ can be summarized as follows:

{\em Perform the static DFS traversal on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices.
%The algorithm for computing a DFS tree of $G+U$ is quite similar
%to the static DFS traversal executed on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices as follows.
%the wherein we grow $L(v)$ for each vertex $v$ lazily and cleverly as follows.
%Consider each element of ${\cal P}\cup{\cal T}$ as a {\em super} vertex.
Visiting a super vertex $v^*$ by the algorithm involves extracting an ancestor-descendant path $p_0$ 
%of $T$ is extracted 
from $v^*$ and attaching it to the partially grown DFS tree $T^*$. The remaining part of 
$v^*$ is added back to $\PP \cup \TT$ as {\em new} super vertices.
% maintaining the properties of disjoint tree partition. 
Thereafter, the reduced adjacency list of the vertices on path $p_0$ is computed using the data structure
$\DD$. The algorithm then continues to find the next super vertex using the reduced adjacency lists. }


%The algorithm for computing a DFS tree of $G+U$ is quite similar
%to the static DFS traversal executed on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices as follows.
%the wherein we grow $L(v)$ for each vertex $v$ lazily and cleverly as follows.
%Consider each element of ${\cal P}\cup{\cal T}$ as a {\em super} vertex.
%Visiting a super vertex $v^*$ by the algorithm involves extracting an ancestor-descendant path $p_0$ 
%of $T$ is extracted 
%from $v^*$ and attaching it to the partially grown DFS tree $T^*$. The remaining part of 
%$v^*$ is added back to $\PP \cup \TT$ as {\em new} super vertices.
% maintaining the properties of disjoint tree partition. 
%Thereafter, the reduced adjacency list of the vertices on path $p_0$ is computed using the data structure
%$\DD$. The algorithm then continues to find the next super vertex using the reduced adjacency lists. 



%Our aim is to bound the total number of queries done between the elements of $\PP\cup \TT$
%and the paths ($p_0$) attached to $T^*$ throughout the algorithm. In order to achieve this one of the
%crucial point is that the number of paths in $\PP$ is always bounded by $|U|$.
% (where $k$ is the size of
%update set $U$). 
%In the next section we see a simple method of initializing disjoint tree partitioning, 
%when all the vertices of the graph except root are unvisited.



%wherein we grow $L(v)$ for 
%vertices lazily and cleverly.  as follows.
 %While computing the DFS tree of $G+U$, our algorithm tries to {\em preserve} 
%$T$ to minimize the computation. 

%The entire algorithm can be seen as the static DFS algorithm executed on the graph 
%with elements of ${\cal P}\cup{\cal T}$ as its {\em super} vertices wherein we grow $L(v)$ for 
%vertices lazily and cleverly. 
%It performs one of the following two steps 
%depending upon whether the next super vertex traversed is a subtree or a path 
%in the partition ${\cal P} \cup {\cal T}$. 
%\begin{enumerate}
%\item
%If the next super vertex is a path $p(x,y)\in {\cal P}$, let $v\in p$ be the 
%vertex which is visited first. 
%Exploiting flexibility of DFS, we traverse from $v$ to $x$ and thus add 
%(hence preserve) path $p(v,x)$ to $T^*$. The untraversed part of $p(x,y)$
%is added to the ${\cal P}$.
%For each vertex $w$ of the newly added path $p(v,x)$, we compute $L(w)$
%by exploiting components property as follows.
%\begin{itemize}
%\item 
%For each tree $\tau \in {\cal T}$, among all edges incident on $\tau$ from
%$path(v,x)$, let $(w,z)$ be the edge such that $w\in path(v,x)$ is nearest to
%$x$ on $path(v,x)$. We insert edge $(w,z)$ to $L(w)$.
%\item 
%For each vertex $w \in path(v,x)$ and every $p\in {\cal P}$, 
%among potentially many edges incident on $w$ from $p$, we add just one edge. 
%\end{itemize}
%In order to perform these two steps, we employ the data structure 
%${\cal D}$. The efficiency of our dynamic algorithm relies heavily on
%this data structure. Its construction employs a novel combination of 
%two well known techniques, namely, heavy-light decomposition and suitably 
%augmented segment tree. 

%\item
%If the next super vertex is a subtree $\tau\in {\cal T}$, let $v\in \tau$
%be the vertex which is visited first. Then, exploiting flexibility of DFS, 
%we traverse the path from $v$ to the root of $\tau$ and add
%it to $T^*$. 
%All the subtrees hanging from this path get added to the pool of ${\cal T}$.
%The components property is now used on this preserved path in the
%same way as in the previous case. 
%\end{enumerate}

%Figure \ref{figure:overview-of-dfs-on-supernodes} provides an illustration of
%this clever DFS traversal on the super vertices of ${\cal P} \cup {\cal T}$.
%Note that our notion of super vertices is for the sake of understanding only.
%An element of $\PP \cup \TT$ representing a super vertex may disintegrate 
%during the algorithm as evident from 
%Figure \ref{figure:overview-of-dfs-on-supernodes}.


%\begin{figure}[!ht]
%\includegraphics[width=\linewidth]{Figures/overview_eg2.pdf}
%\caption{ (i) Initially $\PP$ and $\TT$ both consists of single super
%vertices. (ii) From them $path(e,a)$ and $path(q,n)$ are extracted and 
%attached to $T^*$. The unvisited segments are added back to $\TT$ and 
%$\PP$. (iii) From each unvisited component only lowest edge on $T^*$ is
%required (i.e. $(g,d)$, $(k,b)$ and $(s,q)$).
%}
%\label{figure:overview-of-dfs-on-supernodes}
%\end{figure}


%While building the DFS tree for $G+U$ as sketched above, the partition 
%${\cal P} \cup {\cal T}$ evolves as the algorithm proceeds. Note that the 
%number of paths in ${\cal P}$ remains bounded by $|U|$, though a single 
%path may break and appear multiple times. The number of edges added to 
%$L(v),\forall v\in V$ 
%during the algorithm remain bounded by $O(nk^*)$, where $k^*$ is 
%the number of paths added to $\PP$ during the entire algorithm. Notice that 
%$k^*$ can be much larger than $|U|$ because the DFS traversal may enter
%a path many times during the algorithm. In order to limit $k^*$ we use 
%the technique of {\em path halving} : whenever the DFS enters a path 
%$p\in {\cal P}$, we traverse to the farther end of the path so that the 
%length of the untraversed portion of $p$, to be placed back into ${\cal P}$, 
%is always at most half of $p$. This limits the value of $k^*$ to 
%$O(|U|\log n)$. Similar idea was also used by Aggarwal and Anderson 
%\cite{AggarwalA88} in the parallel algorithm for computing DFS tree in 
%undirected graphs. 

\end{comment}

==> New folder/overview2.tex <==
\section{Handling multiple updates - Overview}
\label{sec:Overview2}
DFS tree can be computed in $\tilde{O}(n)$ time after a single update in the graph, by reducing it to Procedure \ref{alg:re-root}.
However, the same procedure cannot be directly applied to handle a sequence of updates because of the following reason.
The efficiency of Procedure \ref{alg:re-root} crucially depends on the data structure $\cal D$ which is built using the DFS tree $T$ of the original graph.
Thus, when the DFS tree is updated, we are required to rebuild $\cal D$ for the updated tree.
Now, rebuilding $\cal D$ is highly inefficient because it requires $O(m\log n)$ time.  
Thus, in order to handle a sequence of updates, our aim is to use the same $\cal D$ for handling multiple updates,
without having to rebuild it after every update. We now give an overview of the algorithm that reports the DFS tree 
after a set $U$ of updates. %, using the data structure $\cal D$ built on $T$. 

%
%
%%The rerooting procedure can efficiently compute the DFS tree after an update. 
%However, it employs the data structure $\cal D$ which has to be rebuilt whenever the DFS tree is updated.
%Rebuilding $\cal D$ after every update is not feasible as it requires $O(m\log n)$ time.  
%Thus, in order to handle a sequence of updates, our aim is to use $\cal D$ for handling multiple updates together,
%without having to rebuild $\cal D$ after every update. We now describe how to report the DFS tree after 
%a set $U$ of updates, using the data structure $\cal D$ built on the DFS tree $T$ of the original graph. 
%%This gives a fault tolerant algorithm for the problem described as follows.

%Since we cannot rebuild it after 
%every update, a sequence of updates our aim is to handle multiple updates together without having to rebuild the data structure after every update.
%This gives a fault tolerant algorithm for the problem described as follows.
%
%
%However, the time required to build the data structure $\cal D$ is $O(m\log n)$, hence it cannot be rebuild after every update in the DFS tree. 
%Thus in order to handle a sequence of updates our aim is to handle multiple updates together without having to rebuild the data structure after every update.
%This gives a fault tolerant algorithm for the problem described as follows.

In case of a single update, all the edges reported by $\cal D$ are added to the final DFS tree $T^*$.
However, while handling multiple updates, we use $\cal D$ to build {\em reduced adjacency lists} for vertices of the graph, such that the
DFS traversal of the graph using these {\em sparser} lists gives the DFS tree of the updated graph. 
%Now, Instead of querying just the edges required to be added to $T^*$ we build a {\em reduced adjacency list} for the graph such that 
%DFS traversal using these sparser lists gives the DFS tree of the updated graph.
%The components property is exploited to compute these reduced adjacency lists for building a DFS tree as follows.
Now, the data structure $\cal D$ finds the lowest/highest edge from a subtree of $T$ to an ancestor-descendant path of $T$.
Thus, in order to employ $\cal D$ to report DFS tree of $G+U$, we need to ensure that the queried subtrees and paths 
do not contain any failed edges or vertices from $U$. 
%Recall that in Procedure \ref{alg:re-root}, all the edges reported by $\cal D$ are added to the final DFS tree $T^*$.
%However, while handling multiple updates, we use $\cal D$ to build a {\em reduced adjacency list} for the graph 
%such that, DFS traversal of the graph using these sparser lists gives the DFS tree of the updated graph. 
%%Now, Instead of querying just the edges required to be added to $T^*$ we build a {\em reduced adjacency list} for the graph such that 
%%DFS traversal using these sparser lists gives the DFS tree of the updated graph.
%%The components property is exploited to compute these reduced adjacency lists for building a DFS tree as follows.
%Further, recall that the data structure $\cal D$ can answer queries from a subtree of $T$ to an ancestor-descendant path of $T$.
%Thus, in order to employ the data structure $\cal D$ to report the DFS tree of $G+U$,
%we compute a partitioning of $T$ into a disjoint collection of ancestor-descendant paths and subtrees of $T$,
%such that none of these subtrees and paths contain any failed edge or vertex. 
Hence, for any set $U$ of updates, we compute a partitioning of $T$ into 
%Now, consider a set $U$ of updates, we compute a partitioning of $T$ into 
a disjoint collection of ancestor-descendant paths and subtrees
such that none of these subtrees and paths contain any failed edge or vertex. 
An important property of this partitioning is that there are no edges from $G$ lying between
any two subtrees in this partitioning. We refer to this partitioning as a {\em disjoint tree partitioning}.
Note that this partitioning depends only upon  the vertex and edge failures present 
in the set $U$.

Recall that during the DFS traversal we need to find the lowest edge from each component $C$ of the unvisited graph.
It turns out that any component $C$ can be represented as a union of subtrees and ancestor-descendant paths of the original DFS tree $T$. 
%Furthermore, there exists a data structure $\DD$ that can efficiently report the lowest edge from the subtrees and the ancestor-descendant paths to $p_0$.
The components property can now be employed to compute the reduced adjacency lists of the vertices of the graph as follows.
%Thus we employ the components property to 
We just find the lowest edge from each of the subtrees and the ancestor-descendant paths to $T^*$ by querying the data structure $\DD$.
Let this edge be $(x,y)$ where $x\in T^*$ and $y\in C$. We can just add $y$ to the reduced adjacency list $L(x)$ of $x$.
Since the components property ensures the remaining edges to $T^*$ can be ignored, the DFS traversal would thus consider all possible 
candidates for the lowest edge from every component $C$ to $T^*$.
Let the initial disjoint tree partitioning consist of a set of ancestor-descendant paths ${\cal P}$ 
and a set of subtrees ${\cal T}$. The algorithm for computing a DFS tree of $G+U$ can be summarized as follows:

{\em Perform the static DFS traversal on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices.
%The algorithm for computing a DFS tree of $G+U$ is quite similar
%to the static DFS traversal executed on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices as follows.
%the wherein we grow $L(v)$ for each vertex $v$ lazily and cleverly as follows.
%Consider each element of ${\cal P}\cup{\cal T}$ as a {\em super} vertex.
Visiting a super vertex $v^*$ by the algorithm involves extracting an ancestor-descendant path $p_0$ 
%of $T$ is extracted 
from $v^*$ and attaching it to the partially grown DFS tree $T^*$. The remaining part of 
$v^*$ is added back to $\PP \cup \TT$ as {\em new} super vertices.
% maintaining the properties of disjoint tree partition. 
Thereafter, the reduced adjacency lists of the vertices on path $p_0$ are computed using the data structure
$\DD$. The algorithm then continues to find the next super vertex using the reduced adjacency lists and so on. }



\begin{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 14Nov Version %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Overview}
\label{sec:Overview}
Static DFS traversal explores each edge in the graph and thus takes $\Theta(m+n)$ time. 
In order to compute the DFS tree for $G+U$ in $o(m)$ time, the aim is 
to explore only a {\em small} subset of neighbors $L(v)\subseteq N(v)$ of every vertex $v$. 
For this purpose, 
%DFS traversal has the following flexibility : when the traversal reaches  a vertex, say $v$, the next vertex 
%to be traversed can be {\em any} unvisited neighbor of $v$. 
%In order to compute a DFS tree for $G+U$ efficiently, our algorithm exploits this flexibility,
%the original DFS tree $T$, and the following property of DFS traversal.
we exploit the flexibility inherent in DFS traversal 
and an important property. The flexibility of DFS is that once traversal reached a 
vertex $v$, the next vertex to be traversed can be any one among its unvisited 
neighbors. We also exploit the following property of DFS traversal.
%Following We now state the important property of DFS traversal.


\begin{figure}[!hb]
\centering
\includegraphics[width=0.35\linewidth]{Figures/components2.pdf}
\caption{Edges $e_1'$ as well as $e_2'$ can be ignored during the DFS traversal.}
\label{fig:component-property}
\end{figure}

\begin{lemma}[Components Property]
\label{lemma:L()}
%Let $v$ be a vertex that any DFS traversal is visiting currently and $T^*$ be the partially grown DFS tree. 
Let $T^*$ be the partially grown DFS tree and $v$ be the vertex currently visited. 
Let $C$ be any connected component in the subgraph induced by the unvisited vertices.  Suppose two edges $e$ and $e'$ from $C$
are incident respectively on $v$ and some ancestor (not necessarily proper) $w$ of $v$ in $T^*$. Then it is sufficient to 
consider only $e$ during the rest of the DFS traversal, i.e., the edge $e'$ need not  be scanned. (Refer to Figure \ref{fig:component-property}).
\end{lemma}

Skipping $e'$ during the DFS traversal, as stated in the components property, is justified because $e'$ will appear
as a back edge in the resulting DFS tree. 
%Let us now understand how this property can be used to handle a single update in a graph. %, reporting the resulting DFS tree in $\tilde{O}(n)$ time.
In order to have a deeper insight of the components property let us consider a simpler update.
Consider the failure of a single edge $(b,f)$ (refer to Figure \ref{figure:overview-failure-eg} (i)).
Exploiting the flexibility of DFS traversal, we can assume a stage in the DFS traversal of $G\backslash \{(b,f)\}$ where
the partial DFS tree $T^*$ is $T\backslash T(f)$. Note that the unvisited graph is a single connected component
containing the vertices in $T(f)$. Now, using components property we find only the lowest edge from $T(f)$ on $path(e,r)$
($(k,b)$ in Figure \ref{figure:overview-failure-eg} (ii)). Hence entering the component represented by the vertices of $T(f)$,
the DFS traversal rebuilds the DFS tree of the subgraph induced by $T(f)$ which is now rooted at $k$. 
We now describe how this rerooting can be performed recursively to report the resulting DFS tree in $\tilde{O}(n)$ time.


\begin{figure}[!ht]
\centering
\includegraphics[width=.8\linewidth]{Figures/overview_failure_eg3.pdf}
\caption{ (i) Failure of edge $(b,f)$. 
(ii) Partial DFS tree $T^*$ with unvisited graph $T(f)$, component property allows us to neglect $(a,l)$.
(iii) Augmented $path(k,f)$ to $T^*$, components property allows us to neglect $(l,k)$.
(iv) Final DFS tree of $G\backslash \{(b,f)\}$.
}
\label{figure:overview-failure-eg}
\end{figure}

\subsection*{Rerooting a DFS tree}
Given a DFS tree (or its subtree $T(f)$) originally rooted at $r_0$ (here $f$), the aim is to rebuild this DFS tree which is now rooted at 
some vertex $r'$ (here $k$). The traversal first enters the component using $r'$ and traverses the path to the root of this DFS tree $r_0$.
Now, the subtrees hanging from $path(r',r_0)$ forms the components of the unvisited graph ($T(h)$ and $T(l)$ in Figure \ref{figure:overview-failure-eg} (iii)). 
This is because presence of any edge between these subtrees would imply a cross edge in the original DFS tree. 
Using the components property we know that for each of these subtrees (say $T_i$) we find the lowest edge from $T_i$ to $path(r',r_0)$.
Note that since $path(r',r_0)$ is reversed in $T^*$ as compared to $path(r_0,r')$ in $T$, 
it is equivalent to find the highest edge $e_i$ from $T_i$ on $path(r_0,r')$ in $T$.
Now, each $T_i$ would be rerooted independent of each other on the new root (end point of $e_i$ in $T_i$) when the DFS traversal enters 
$T_i$ using the edge $e_i$. This process continues using recursively rerooting subtrees of $T$ until every vertex is visited. 
 
The total time required to reroot a DFS tree is thus dependent on how efficiently we can find the lowest/highest edge from a subtree of $T$
to some path in $T$. In section \ref{sec:data-structure} we describe a data structure $\cal D$ that preprocesses the graph $G$ and the DFS tree $T$
in $O(m\log n)$ time to allow us to find such an edge in $O(\log ^3 n)$ time.
The total edges processed by our algorithm are limited to the ones returned by our data structure, which eventually becomes a part of the new DFS tree $T^*$.
These edges are limited to size of $T'$, hence the total time taken by our algorithm to rebuild $T'$ is $O(|T'|\log^3 n)$ time. Thus we have the following lemma.  

\begin{lemma}
An undirected graph can be preprocessed to build a data structure in $O(m \log n)$ time such that 
any subtree $T'$ of the DFS tree can be rebuild to be rooted at some vertex in $T'$ in $O(|T'| \log^3 n)$ time.
\label{lemm:reroot}
\end{lemma}

Thus the DFS tree can be rebuilt after an edge deletion in $\tilde{O}(n)$ time.
Further the reader may note that several other kinds of updates in the graph as insertion of an edge, insertion/deletion of a vertex etc.
can also be reduced to this simple rerooting procedure.
However, the time required to build the data structure $\cal D$ is $O(m\log n)$, hence it cannot be rebuild after every update in the DFS tree. 
Thus in order to handle a sequence of updates our aim is to handle multiple updates together without having to rebuild the data structure after every update.
This gives a fault tolerant algorithm for the problem described as follows.

\subsection*{Fault tolerant DFS}
Instead of querying just the edges required to be added to $T^*$ we build a {\em reduced adjacency list} for the graph such that 
DFS traversal using these sparser lists gives the DFS tree of the updated graph.
%The components property is exploited to compute these reduced adjacency lists for building a DFS tree as follows.
Consider a set $U$ of updates, we compute a partitioning of $T$ into 
a disjoint collection of ancestor-descendant paths and subtrees
such that none of these subtrees and paths contain any failed edge or vertex. 
An important property of this partitioning is that there are no edges from $G$ lying between
any two subtrees in this partitioning. We refer to this partitioning as a {\em disjoint tree partitioning}.
In fact, this partitioning depends upon only the vertex and edge failures in the set $U$.

Recall that during the DFS traversal we need to find the lowest edge from each component $C$ of the unvisited graph.
It turns out that each component $C$ can be represented as a union of subtrees and ancestor-descendant paths of the original DFS tree $T$. 
%Furthermore, there exists a data structure $\DD$ that can efficiently report the lowest edge from the subtrees and the ancestor-descendant paths to $p_0$.
The components property can now be employed to compute the reduced adjacency lists of the graph as follows.
%Thus we employ the components property to 
We just find the lowest edge from each of the subtrees and the ancestor-descendant paths to $T^*$ by querying the data structure $\DD$.
Let this edge be $(x,y)$ where $x\in T^*$ and $y\in C$. We can just add $y$ to the reduced adjacency list $L(x)$ of $x$.
Since components property ensures the remaining edges to $T^*$ can be ignored, the DFS traversal would thus consider all possible 
candidates for the lowest edge from $C$ to $T^*$.
Let the initial disjoint tree partitioning consists of a set of ancestor-descendant paths ${\cal P}$ 
and a set of subtrees ${\cal T}$. The algorithm for computing a DFS tree of $G+U$ can be summarized as follows:

{\em Perform the static DFS traversal on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices.
%The algorithm for computing a DFS tree of $G+U$ is quite similar
%to the static DFS traversal executed on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices as follows.
%the wherein we grow $L(v)$ for each vertex $v$ lazily and cleverly as follows.
%Consider each element of ${\cal P}\cup{\cal T}$ as a {\em super} vertex.
Visiting a super vertex $v^*$ by the algorithm involves extracting an ancestor-descendant path $p_0$ 
%of $T$ is extracted 
from $v^*$ and attaching it to the partially grown DFS tree $T^*$. The remaining part of 
$v^*$ is added back to $\PP \cup \TT$ as {\em new} super vertices.
% maintaining the properties of disjoint tree partition. 
Thereafter, the reduced adjacency list of the vertices on path $p_0$ is computed using the data structure
$\DD$. The algorithm then continues to find the next super vertex using the reduced adjacency lists. }






\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUBMITTED SODA VERSION %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Static DFS traversal has to explore each edge and thus needs $\Theta(m+n)$ 
%time. In order to compute the DFS tree for $G+U$ in $o(m)$ time, the aim is 
%to explore only a {\em small} subset of neighbors $L(v)\subseteq N(v)$ of every 
%vertex $v$. For this purpose, 
DFS traversal has the following flexibility : when the traversal reaches  a vertex, say $v$, the next vertex 
to be traversed can be {\em any} unvisited neighbor of $v$. 
In order to compute a DFS tree for $G+U$ efficiently, our algorithm exploits this flexibility,
the original DFS tree $T$, and the following property of DFS traversal.
%
%We exploit the flexibility inherent in DFS traversal 
%and an important property. The flexibility of DFS is that once traversal reached a 
%vertex $v$, the next vertex to be traversed can be any one among its unvisited 
%neighbors of $v$. We now state the important property of DFS traversal.
%


\begin{figure}[!hb]
\centering
\includegraphics[width=0.35\linewidth]{Figures/components2.pdf}
\caption{Edges $e_1'$ as well as $e_2'$ can be ignored during the DFS traversal.}
\label{fig:component-property}
\end{figure}

\begin{lemma}[Components Property]
\label{lemma:L()}
%Let $v$ be a vertex that any DFS traversal is visiting currently and $T^*$ be the partially grown DFS tree. 
Let $T^*$ be the partially grown DFS tree and $v$ be the vertex currently visited. 
Let $C$ be any connected component in the subgraph induced by the unvisited vertices.  Suppose two edges $e$ and $e'$ from $C$
are incident respectively on $v$ and some ancestor (not necessarily proper) $w$ of $v$ in $T^*$. Then it is sufficient to 
consider only $e$ during the rest of the DFS traversal, i.e., the edge $e'$ need not  be scanned. (Refer to Figure \ref{fig:component-property}).
\end{lemma}

Skipping $e'$ during the DFS traversal, as stated in the components property, is justified because $e'$ will appear
as a back edge in the resulting DFS tree.
%-------------------8July  begins-------
%To understand the main intuition behind the components property, consider the instance when 
%DFS traversal reaches a vertex $v$. Let $H$ be the unvisited graph at this instance, and 
%$(v,x)$ be the first edge scanned by $v$ that is incident to it from component $C$.
%As a result $x$ becomes a child of $v$. Now note that the DFS traversal on reaching $x$ is like 
%a fresh DFS from $x$ in the graph $H$. Thus, at the time when DFS traversal finishes for
%vertex $x$, all the vertices that were reachable from $x$ in $H$ (this is essentially 
%set $C$) lie in subtree under $x$.
%Let $e'=(w,x')$ where $w$ an ancestor of $v$ and $x' \in C$
%Since w is an ancestor of x, we have that e' is a back edge in the final DFS tree.
%-----------------8-July ends----------
%
%
% Hence, from each component we only need to find the lowest (??) edge (say $(u,v)$ where $u\in T^*$)
% incident on the partially build DFS tree and add $v$ to the reduced adjacency list $L(u)$ of $u$.
%
% Consider a path $p_0$ in the partially built DFS tree $T^*$ for whose vertices we need to 
% compute reduced adjacency list. By Lemma \ref{lemma:L()} from each component $C$ of the unvisited 
% graph we only need to find a lowest edge incident on $p_0$ (say $(u,v)$ where $u\in p_0$, and $v\in C$)
% and add $v$ to the reduced adjacency list $L(u)$ of $u$.
% 
The components property can be exploited to compute reduced adjacency lists of small size for building a DFS tree as follows.
Let $p_0$ be the path from the root to $v$ in the partially built DFS tree $T^*$.
%The components property implies the existence of reduced adjacency lists of small size as follows. Let $p_0$ be the path
%from the root to $v$ in the partially built DFS tree $T^*$.
% for whose vertices we need to 
%compute reduced adjacency list. By Lemma \ref{lemma:L()} 
From each component $C$ of the unvisited graph, we only need to find an edge incident to the lowest vertex on $p_0$.
Let this edge be $(x,y)$ where $x\in p_0$ and $y\in C$. We can just add $y$ to the reduced adjacency list $L(x)$ of $x$ and ignore
all other edges incident from $C$ to $p_0$.
%
% Consider a path $p_0$ in the partially built DFS tree $T^*$ for whose vertices we need to 
% compute reduced adjacency list. By Lemma \ref{lemma:L()} from each component $C$ of the unvisited 
% graph we only need to find a lowest vertex on $p_0$ adjacent to $C$, say $u$,
% and add a vertex from $N(u)\cap C$ to reduced adjacency list $L(u)$.
%
% In order to understand our algorithm we first consider the stack based standard DFS algorithm.
% In it whenever a vertex $u$ is visited for the first time by the traversal it is pushed 
% into stack $S$, and the whole adjacency list of $u$ is scanned before it is popped out. 
% In order to compute the DFS tree for a graph after a given set of updates we perform a
% modified DFS traversal of it as follows. Whenever a vertex $u$ is visited for the first 
% time, then instead of just attaching $u$ to the tree, we extract a path $p_0$ (starting 
% from $u$) from the unvisited graph an attach it to partially built DFS tree. 
% We exploit here the flexibility of DFS traversal that on reaching a vertex $u$ it can 
% follow any arbitrary path in the unvisited graph.
% We mark the vertices of $p_0$ as visited and also push them in the stack.
% Next we compute the reduced adjacency list of vertices belonging to path $p_0$.
% For each component $C$ in the unvisited graph we ensure that if $w$ is the 
% lowest vertex on path $p_0$ (i.e. vertex farthest from root) which is adjacent to $C$,
% then at least one vertex from $N(w)\cap C$ is added to set $L(w)$.
% It turns out that the reduced adjacency lists constructed in this fashion are sufficient
% to be scanned in order to obtain a valid DFS tree.
%
%
%The task of computing the reduced adjacency lists efficiently is accomplished
%using the original DFS tree $T$ as follows.
However, as the reader may also observe, maintaining the connected components 
of the unvisited graph and obtaining the lowest edge incident from each of them to $p_0$ is a non-trivial task. 
Nevertheless, we are able to accomplish this task by exploiting the original DFS tree $T$ of $G$ as follows. 

%----------commented on 13October
%We compute and maintain a partitioning of the unvisited graph into 
%a disjoint collection of ancestor-descendant paths and subtrees of $T$  
%such that none of these subtrees and paths contain any failing edge or vertex. 
%We refer to this partitioning as a {\em disjoint tree partitioning}.
%An important property of this partitioning is that there are no edges from $G+U$ lying between
%any two subtrees in ${\cal T}$. 
%It turns out that each component $C$ of the unvisited graph during a DFS traversal can be represented 
%as a union of  subtrees and ancestor-descendant paths of the original DFS tree $T$. 
%Furthermore, there exists a data structure $\DD$ that can efficiently report the lowest edge from the subtrees and the ancestor-descendant paths to $p_0$.
%The lowest edges from the subtrees and the ancestor-descendant paths is then obtained by querying the %data structure $\DD$.

For a given set $U$ of updates, we compute a partitioning of $T$ into 
a disjoint collection of ancestor-descendant paths and subtrees
such that none of these subtrees and paths contain any failed edge or vertex. 
An important property of this partitioning is that there are no edges from $G$ lying between
any two subtrees in ${\cal T}$. We refer to this partitioning as a {\em disjoint tree partitioning}.
Note that this partitioning depends upon only the vertex and edge failures in the set $U$.
It turns out that each component $C$ of the unvisited graph during a DFS traversal can be represented 
as a union of subtrees and ancestor-descendant paths of the original DFS tree $T$. 
%Furthermore, there exists a data structure $\DD$ that can efficiently report the lowest edge from the subtrees and the ancestor-descendant paths to $p_0$.
The lowest edges from the subtrees and the ancestor-descendant paths can be obtained by querying the data structure $\DD$.

%With insights from the disjoint tree partitioning and the component property at its core, 
%our algorithm now exploits the flexibility of the DFS traversal to compute the DFS tree of $G+U$ as %follows.
Let the initial disjoint tree partitioning consists of a set of ancestor-descendant paths ${\cal P}$ 
and a set of subtrees ${\cal T}$. The algorithm for computing a DFS tree of $G+U$ can be summarized as follows:

{\em Perform the static DFS traversal on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices.
%The algorithm for computing a DFS tree of $G+U$ is quite similar
%to the static DFS traversal executed on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices as follows.
%the wherein we grow $L(v)$ for each vertex $v$ lazily and cleverly as follows.
%Consider each element of ${\cal P}\cup{\cal T}$ as a {\em super} vertex.
Visiting a super vertex $v^*$ by the algorithm involves extracting an ancestor-descendant path $p_0$ 
%of $T$ is extracted 
from $v^*$ and attaching it to the partially grown DFS tree $T^*$. The remaining part of 
$v^*$ is added back to $\PP \cup \TT$ as {\em new} super vertices.
% maintaining the properties of disjoint tree partition. 
Thereafter, the reduced adjacency list of the vertices on path $p_0$ is computed using the data structure
$\DD$. The algorithm then continues to find the next super vertex using the reduced adjacency lists. }


%The algorithm for computing a DFS tree of $G+U$ is quite similar
%to the static DFS traversal executed on the graph with the elements of ${\cal P}\cup{\cal T}$ as the {\em super} vertices as follows.
%the wherein we grow $L(v)$ for each vertex $v$ lazily and cleverly as follows.
%Consider each element of ${\cal P}\cup{\cal T}$ as a {\em super} vertex.
%Visiting a super vertex $v^*$ by the algorithm involves extracting an ancestor-descendant path $p_0$ 
%of $T$ is extracted 
%from $v^*$ and attaching it to the partially grown DFS tree $T^*$. The remaining part of 
%$v^*$ is added back to $\PP \cup \TT$ as {\em new} super vertices.
% maintaining the properties of disjoint tree partition. 
%Thereafter, the reduced adjacency list of the vertices on path $p_0$ is computed using the data structure
%$\DD$. The algorithm then continues to find the next super vertex using the reduced adjacency lists. 



%Our aim is to bound the total number of queries done between the elements of $\PP\cup \TT$
%and the paths ($p_0$) attached to $T^*$ throughout the algorithm. In order to achieve this one of the
%crucial point is that the number of paths in $\PP$ is always bounded by $|U|$.
% (where $k$ is the size of
%update set $U$). 
%In the next section we see a simple method of initializing disjoint tree partitioning, 
%when all the vertices of the graph except root are unvisited.



%wherein we grow $L(v)$ for 
%vertices lazily and cleverly.  as follows.
 %While computing the DFS tree of $G+U$, our algorithm tries to {\em preserve} 
%$T$ to minimize the computation. 

%The entire algorithm can be seen as the static DFS algorithm executed on the graph 
%with elements of ${\cal P}\cup{\cal T}$ as its {\em super} vertices wherein we grow $L(v)$ for 
%vertices lazily and cleverly. 
%It performs one of the following two steps 
%depending upon whether the next super vertex traversed is a subtree or a path 
%in the partition ${\cal P} \cup {\cal T}$. 
%\begin{enumerate}
%\item
%If the next super vertex is a path $p(x,y)\in {\cal P}$, let $v\in p$ be the 
%vertex which is visited first. 
%Exploiting flexibility of DFS, we traverse from $v$ to $x$ and thus add 
%(hence preserve) path $p(v,x)$ to $T^*$. The untraversed part of $p(x,y)$
%is added to the ${\cal P}$.
%For each vertex $w$ of the newly added path $p(v,x)$, we compute $L(w)$
%by exploiting components property as follows.
%\begin{itemize}
%\item 
%For each tree $\tau \in {\cal T}$, among all edges incident on $\tau$ from
%$path(v,x)$, let $(w,z)$ be the edge such that $w\in path(v,x)$ is nearest to
%$x$ on $path(v,x)$. We insert edge $(w,z)$ to $L(w)$.
%\item 
%For each vertex $w \in path(v,x)$ and every $p\in {\cal P}$, 
%among potentially many edges incident on $w$ from $p$, we add just one edge. 
%\end{itemize}
%In order to perform these two steps, we employ the data structure 
%${\cal D}$. The efficiency of our dynamic algorithm relies heavily on
%this data structure. Its construction employs a novel combination of 
%two well known techniques, namely, heavy-light decomposition and suitably 
%augmented segment tree. 

%\item
%If the next super vertex is a subtree $\tau\in {\cal T}$, let $v\in \tau$
%be the vertex which is visited first. Then, exploiting flexibility of DFS, 
%we traverse the path from $v$ to the root of $\tau$ and add
%it to $T^*$. 
%All the subtrees hanging from this path get added to the pool of ${\cal T}$.
%The components property is now used on this preserved path in the
%same way as in the previous case. 
%\end{enumerate}

%Figure \ref{figure:overview-of-dfs-on-supernodes} provides an illustration of
%this clever DFS traversal on the super vertices of ${\cal P} \cup {\cal T}$.
%Note that our notion of super vertices is for the sake of understanding only.
%An element of $\PP \cup \TT$ representing a super vertex may disintegrate 
%during the algorithm as evident from 
%Figure \ref{figure:overview-of-dfs-on-supernodes}.


%\begin{figure}[!ht]
%\includegraphics[width=\linewidth]{Figures/overview_eg2.pdf}
%\caption{ (i) Initially $\PP$ and $\TT$ both consists of single super
%vertices. (ii) From them $path(e,a)$ and $path(q,n)$ are extracted and 
%attached to $T^*$. The unvisited segments are added back to $\TT$ and 
%$\PP$. (iii) From each unvisited component only lowest edge on $T^*$ is
%required (i.e. $(g,d)$, $(k,b)$ and $(s,q)$).
%}
%\label{figure:overview-of-dfs-on-supernodes}
%\end{figure}


%While building the DFS tree for $G+U$ as sketched above, the partition 
%${\cal P} \cup {\cal T}$ evolves as the algorithm proceeds. Note that the 
%number of paths in ${\cal P}$ remains bounded by $|U|$, though a single 
%path may break and appear multiple times. The number of edges added to 
%$L(v),\forall v\in V$ 
%during the algorithm remain bounded by $O(nk^*)$, where $k^*$ is 
%the number of paths added to $\PP$ during the entire algorithm. Notice that 
%$k^*$ can be much larger than $|U|$ because the DFS traversal may enter
%a path many times during the algorithm. In order to limit $k^*$ we use 
%the technique of {\em path halving} : whenever the DFS enters a path 
%$p\in {\cal P}$, we traverse to the farther end of the path so that the 
%length of the untraversed portion of $p$, to be placed back into ${\cal P}$, 
%is always at most half of $p$. This limits the value of $k^*$ to 
%$O(|U|\log n)$. Similar idea was also used by Aggarwal and Anderson 
%\cite{AggarwalA88} in the parallel algorithm for computing DFS tree in 
%undirected graphs. 

\end{comment}

==> New folder/partitioning.tex <==
%\subsection{Disjoint Tree Partitioning}
\section{Disjoint Tree Partitioning}
\label{sec:partition}

We formally define disjoint tree partitioning as follows.

% Given a set $S$ of vertices 
%We first formally define disjoint tree partitioning as follows.

\begin{definition}%[Disjoint tree partitioning of a set]
Given a DFS tree $T$ of an undirected graph $G$ and a set $U$ of failed vertices and edges,
let $A$ be a vertex set in $G+U$. The disjoint tree partitioning defined by $A$ 
is a partition of the subgraph of $T$ induced by $A$ into
%a disjoint tree partitioning of any vertex set $A$ in $G+U$ is a partition of the set $A$ into 
\begin{enumerate}
\item A set of paths $\PP$ such that
(i) each path in $\PP$ is an ancestor-descendant path in $T$ and does not contain any deleted
edge or vertex, and (ii) $|\PP| \le |U|$.
\item A set of trees $\TT$ such that 
each tree $\tau \in \TT$ is a subtree of $T$ which does not contain any deleted
edge or vertex.
\end{enumerate}
Note that for any $\tau_1,\tau_2\in\TT$, there is no edge between $\tau_1$ and $\tau_2$ because 
$T$  is a DFS tree.
\label{definition:disjoint-tree-partition}
\end{definition}

%\noindent
%{\em Remark:} We have defined $\PP\cup\TT$ as the partition of the vertex set $A$. However,  
%we are actually partitioning the subgraph of $T$ induced by the vertex set $A$.
%it represents the whole paths and subtrees in $\PP$ and $\TT$ respectively (not just the corresponding vertices).

%\noindent
%{\em Remark:} We have defined $\PP\cup\TT$ as the partition of the vertex set $A$. However,  %only for the sake of simplicity. 
%we shall abuse the notation to represent the whole paths and subtrees in $\PP$ and $\TT$ respectively (not just the corresponding vertices).
%{\em Remark:} Since the elements of $\PP$ and $\TT$ are respectively the paths and subtrees of $T$, $\PP\cup\TT$ cannot
%represent a partition of a set of vertices. But we abuse our notation for the sake of simplicity.
% (i) Even though we define $\PP$ and $\TT$ to be partition of vertices of $A$, 
% the sets $\PP$ and $\TT$ represent the complete paths and subtrees respectively.
%$$\PP$ and $\TT$ represents the corresponding paths 
%and tree with  are partitioned 
%For notational convenience let $\PP\cup\TT$ represent the set of all paths in $\PP$ and subtrees
%in $\TT$.
%If the elements of $\PP$, $\TT$ are respectively paths and subtrees, then  cannot
%represent a partition of a set of vertices. But we abuse our notation for sake of simplicity.

%If $(\PP,\TT)$ is a disjoint tree partitioning, then no two subtrees of $\TT$
%can be adjacent to each other. This is because DFS tree does not contain any cross edges.


The disjoint tree partitioning for set $A=V\setminus \{r\}$ can be computed as follows.
Let $V_f$ and $E_f$ respectively denote the set of failed vertices and edges associated with the updates $U$.
We initialize $\PP=\emptyset$ and $\TT=\{T(w)~|~w ~\mbox{is a child of $r$}\}$. We refine the
partitioning by processing each vertex $v\in V_f$ as follows 
(see Figure \ref{figure:disjoint-tree-partition} (i)). 
\begin{itemize}
\item 
%$\bullet$ 
If $v$ is present in some $T'\in \TT$, we add the path from $par(v)$
to the root of $T'$ to $\PP$. We remove $T'$ from $\TT$ and 
add all the subtrees hanging from 
% children of $v$ as well as all the subtrees hanging from 
this path to $\TT$. 
\item 
%$\bullet$ 
If $v$ is present in some path $p\in \PP$, we split $p$ at $v$ into 
two paths. We remove $p$ from $\PP$ and add these two paths to $\PP$.
\end{itemize}
%Note that path to be added may be empty. 
Edge deletions are handled as follows.
We first remove edges from $E_f$ that don't appear in $T$. Processing of 
the remaining edges from $E_f$ is quite similar to the processing of $V_f$
as described above. For each edge $e\in E_f$, just visualize deleting an 
imaginary vertex lying at mid-point of the edge $e$ (see Figure \ref{figure:disjoint-tree-partition} (ii)).
It takes $O(n)$ time to process any $v\in V_f$ and any $e\in E_f$.  

%\begin{wrapfigure}[6]{r}[.5\width+.5\columnsep]{6cm}


\begin{figure}[th]
\centering
\includegraphics[width=\linewidth]{Figures/partitioning_eg3.pdf}
\caption{
Disjoint tree partitioning for $V\setminus \{r\}$:
(i) Initializing $\TT=\{T(a),T(h)\}$ and $\PP=\emptyset$,
(ii) Disjoint tree partition obtained after deleting the vertex $g$.
(iii) Final disjoint tree partition obtained after deleting the edges $(c,d)$ and $(m,n)$.}
\label{figure:disjoint-tree-partition}
\end{figure}


%\begingroup
%\centering
%\includegraphics[width=\linewidth]{Figures/partitioning_eg4.pdf}
%\captionof{figure}{
%Disjoint tree partition for $V\setminus \{r\}$:\newline
%(i) Initializing $\TT=\{T(a),T(h)\}$ and $\PP=\emptyset$,\newline
%(ii) Final disjoint tree partition obtained after deleting vertex $g$ and edges $(c,d)$ and $(m,n)$.\newline}
%\label{figure:disjoint-tree-partition}
%\endgroup


Note that each update can add at most one path %(if the added path is not empty) 
to $\PP$. So the size of $\PP$ is bounded by $|U|$. The fact that $T$ is a DFS tree of $G$ ensures that no two
subtrees in ${\cal T}$ will have an edge between them. So $\PP \cup {\cal T}$
satisfies all the conditions stated in Definition 
\ref{definition:disjoint-tree-partition}. 
%It can also be seen easily that each update can be applied to 
%$\PP\cup \TT$ in $O(n)$ time. Thus the disjoint tree partitioning can be found 
%in $O(nk)$ time.

\begin{lemma}
Given an undirected graph $G$ with a DFS tree $T$ and a set $U$ of failing vertices and edges, 
%(edge and vertex failures), 
we can find a disjoint tree partition of set $V\setminus\{r\}$ 
in $O(n|U|)$ time. 
\label{lemma:partition}
\end{lemma}


==> New folder/prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

%Let $G=(V,E)$ be any given undirected graph on $n=|V|$ vertices and $m=|E|$ edges. 
Let $U$ be any given set of updates. We add a dummy 
vertex $r$ to the given graph in the beginning and connect it to all the
vertices. Our algorithm starts with any arbitrary DFS tree $T$ rooted at 
$r$ in the augmented graph and it maintains a DFS tree rooted at $r$ at
each stage. It can be observed easily that each subtree rooted at any 
child of $r$ is a DFS tree of a connected component of the graph $G+U$.
The following notations will be used throughout the paper.

\begin{itemize}
\itemsep0em 
\item  $T(x):$ The subtree of $T$ rooted at vertex $x$.
\item  $path(x,y):$ Path from the vertex $x$ to the vertex $y$ in $T$.
\item  $dist_T(x,y):$ The number of edges on the path from $x$ to $y$ in $T$.
\item  $LCA(x,y):$ The lowest common ancestor of $x$ and $y$ in tree $T$.
\item  $N(w):$ 
The adjacency list of vertex $w$ in the graph $G+U$.
%The neighbors of vertex $w$ in the adjacency list of $G+U$.
%The neighbors of vertex $w$ in graph $G+U$.
\item  $L(w):$ %The neighbors of vertex $w$ in the reduced adjacency list of $G+U$.
The reduced adjacency list of vertex $w$ in the graph $G+U$.
%The subset of neighbors of $w$ in graph $G+U$ used to build $T^*$ by our algorithm.
%\item Ancestor-Descendant path: A path $p(x,y)$ in $T$ where either $x$ is an ancestor of $y$ in $T$ or vice-versa.
\item $T^*:$~ The DFS tree rooted at $r$ computed by our algorithm for
the graph $G+U$.
\item $par(w):$~ Parent of $w$ in $T^*$.
\end{itemize}

\begin{comment}
\noindent
$\bullet$ $T(x):$ The subtree of $T$ rooted at vertex $x$.\\
$\bullet$ $path(x,y):$ Path from vertex $x$ to vertex $y$ in $T$.\\
$\bullet$ $dist_T(x,y):$ The number of edges on the path from $x$ to $y$ in $T$.\\
$\bullet$ $LCA(x,y):$ The lowest common ancestor of $x$ and $y$ in tree $T$.\\
$\bullet$ $N(w):$ 
The adjacency list of vertex $w$ in the graph $G+U$.\\
%The neighbors of vertex $w$ in the adjacency list of $G+U$.
%The neighbors of vertex $w$ in graph $G+U$.
$\bullet$ $L(w):$ %The neighbors of vertex $w$ in the reduced adjacency list of $G+U$.
The reduced adjacency list of vertex $w$ in the graph $G+U$.\\
%The subset of neighbors of $w$ in graph $G+U$ used to build $T^*$ by our algorithm.
%\item Ancestor-Descendant path: A path $p(x,y)$ in $T$ where either $x$ is an ancestor of $y$ in $T$ or vice-versa.
$\bullet$ $T^*:$~ The DFS tree rooted at $r$ computed by our algorithm for
the graph $G+U$.\\
$\bullet$ $par(w):$~ Parent of $w$ in $T^*$.\\
%\end{itemize}
\end{comment}

A subtree $T'$ is said to be {\em hanging} from a path $p$ if the root $r'$ of $T'$ is a child of some vertex on the path $p$
and $r'$ does not belong to the path $p$. 
Unless stated otherwise, every reference to a path refers to an
%We now define the notion of 
ancestor-descendant path defined as follows:

\begin{definition}[Ancestor-descendant path]
A path $p$ in a DFS tree $T$ is said to be ancestor-descendant path 
if its endpoints have ancestor-descendant relationship in $T$.
\label{definition:anc-des}
\end{definition}

%We maintain a data structure $\DD$ (described in Section \ref{sec:data-structure}) 
%by preprocessing the DFS tree $T$. 
We now state the operations supported by the data structure $\DD$ (complete details of $\DD$ are in Section \ref{sec:data-structure}). 
Let $U$ below refer to a set of updates that consists of vertex and edge deletions only.
For any three vertices $w,x,y\in T$, where $path(x,y)$ is an 
ancestor-descendant path in $T$, the following two queries can be answered using $\DD$ in $O(\log^3 n)$ time.
\begin{enumerate}
\item $Query(w,x,y):$ 
among all the edges from $w$ that are incident on $path(x,y)$ %from $w$ 
in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.

\item $Query(T(w),x,y):$ 
among all the edges from $T(w)$ that are incident on $path(x,y)$ %from
in $G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.
\end{enumerate}



We now describe an important property of a DFS traversal that will be crucially 
used in our algorithm.  

%We keep a data structure $\DD$ (refer to Appendix \ref{sec:data-structure}) 
%defined for the tree $T$ and updates $U$.
%For any three vertices $w,x,y\in T$, the following two queries can be 
%answered using $\DD$ in $O(\log^3 n)$ time.
%\begin{enumerate}
%\item $Query(w,x,y):$ among all edges incident on $path(x,y)$ from $w$ in
%$G+U$, return an edge that is incident nearest to $x$ on $path(x,y)$.

%\item $Query(T(w),x,y):$ among all edges incident on $path(x,y)$ from
%$T(w)$ in $G+U$, return an edge that is incident nearest to $x$ on 
%$path(x,y)$.
%\end{enumerate}

